Online Weighted Degree-Bounded Steiner Networks via Novel Online Mixed Packing/Covering

We design the first online algorithm with poly-logarithmic competitive ratio for the edge-weighted degree-bounded Steiner forest(EW-DB-SF) problem and its generalized variant. We obtain our result by demonstrating a new generic approach for solving mixed packing/covering integer programs in the online paradigm. In EW-DB-SF we are given an edge-weighted graph with a degree bound for every vertex. Given a root vertex in advance we receive a sequence of terminal vertices in an online manner. Upon the arrival of a terminal we need to augment our solution subgraph to connect the new terminal to the root. The goal is to minimize the total weight of the solution while respecting the degree bounds on the vertices. In the offline setting edge-weighted degree-bounded Steiner tree (EW-DB-ST) and its many variations have been extensively studied since early eighties. Unfortunately the recent advancements in the online network design problems are inherently difficult to adapt for degree-bounded problems. In contrast in this paper we obtain our result by using structural properties of the optimal solution, and reducing the EW-DB-SF problem to an exponential-size mixed packing/covering integer program in which every variable appears only once in covering constraints. We then design a generic integral algorithm for solving this restricted family of IPs. We demonstrate a new technique for solving mixed packing/covering integer programs. Define the covering frequency k of a program as the maximum number of covering constraints in which a variable can participate. Let m denote the number of packing constraints. We design an online deterministic integral algorithm with competitive ratio of O(k log m) for the mixed packing/covering integer programs. We believe this technique can be used as an interesting alternative for the standard primal-dual techniques in solving online problems.

==> 2nd_proof_useless/abstract.tex <==
	We initiate the study of
	degree-bounded network design problems in the online setting.
	The degree-bounded Steiner tree problem -- which
	asks for a subgraph with minimum degree that connects a
	given set of vertices -- is perhaps one of the
	most representative problems in this class. This paper
	deals with its well-studied generalization called the
	degree-bounded Steiner forest problem where the connectivity
	demands are represented by vertex pairs that need to be individually connected.
	In the classical online model, the input graph is
	given offline but the demand pairs arrive sequentially
	in online steps. The selected subgraph starts off as the 
	empty subgraph, but has to be augmented to satisfy
	the new connectivity constraint in each online step.
	The goal is to be competitive against an adversary that knows the input in advance.
	
	The standard techniques for solving degree-bounded problems often fall in the category of \textit{iterative} and \textit{dependent} rounding techniques. Unfortunately, these rounding methods are inherently difficult to adapt to an online settings since the underlying fractional solution may change dramatically in between the rounding steps. Indeed, this might be the very reason that despite many advances in the online network design paradigm in the past two decades, the natural family of degree-bounded problems has remained widely open.
	
	In this paper, we design an intuitive greedy-like algorithm that achieves a competitive
	ratio of $O(\log n)$ where $n$ is the number of vertices.
	We show that no (randomized) algorithm can achieve a (multiplicative)
	competitive ratio $o(\log n)$; thus our result is asymptotically tight.
	We further show strong hardness results for the group Steiner tree and
	the edge-weighted variants of degree-bounded connectivity problems.
	
	F{\"u}rer and Raghavachari resolved the offline variant of degree-bounded
	Steiner forest in their paper in SODA'92. Since then, the family of
	degree-bounded network design problems has been extensively studied in the
	literature resulting in the development of many interesting tools and
	numerous papers on the topic.
	We hope that our approach and its dual analysis, paves the way for solving the
	\textit{online} variants of the classical problems in this family of problems.

==> 2nd_proof_useless/lemma.tex <==
\section{Main Lemma}
Before we proceed to the proof of Lemma \ref{main}, we state the following observation as an auxiliary lemma. 
\begin{lemma}\label{aux}
Every tree $T$ with at least 3 vertices can be decomposed into two edge-disjoint trees $T_1$ and $T_2$ such that $|V(T_1)\cap V(T_2)|$ = 1, $E(T)  = E(T_1) \cup E(T_2)$, and $\max\{|V(T_1)|,|V(T_2)|\} \leq \lceil \frac{2}{3} |V(T)|\rceil + 1 $.
\end{lemma}
\begin{proof}
Without loss of generality we assume that the tree is rooted at some vertex. We define the weight of every vertex as the number of vertices in its subtree including itself. Let $v$ be a vertex with the highest depth that has a weight of at least $\lfloor \frac{1}{3} |V(T)| \rfloor$. If we remove vertex $v$ and all the edges incident to $v$ from the tree, none of the remaining connected components would have a size more than $\lceil \frac{2}{3} |V(T)|\rceil + 1 $. 

Now, we start with an empty set $X$ and greedily add the vertices of the connected components to $X$ in descending order of their size until $|X|$ reaches $\lfloor \frac{1}{3} |V(T)| \rfloor$. Therefore $|X|$ contains at least $\lfloor \frac{1}{3} |V(T)| \rfloor$ vertices but its size is no more $\lceil \frac{2}{3} |V(T)|\rceil$. We define $T_1$ as the induced subgraph of $T$ on $\{v\} \cup X$ and $T_2$ as the induced subgraph of $T$ on $V(T) \setminus X$. Since $\lfloor \frac{1}{3} |V(T)| \rfloor \leq |X| \leq \lceil \frac{2}{3} |V(T)|\rceil$ we have $\max\{|V(T_1)|,|V(T_2)|\} \leq \lceil \frac{2}{3} |V(T)|\rceil + 1 $ and both $T_1$ and $T_2$ are trivially connected. Moreover $V(T_1) \cap V(T_2) = \{v\}$ and thus the proof is complete.
\end{proof}

\begin{lemma}\label{main}
Let $G$ be graph, $L$ be a collection of pairs of vertices $(s_1, t_1), (s_2, t_2) \ldots, (s_k, t_k)$ and $F$ be a forest in $G$ connecting every vertex $s_i$ to $v_i$. We say a list of $k-1$ subgraphs $Q = \langle Q_2, Q_3, \ldots, _k\rangle$ is \text{connective} for $\langle G, F, L\rangle$ if for every  $1 \leq i \leq k$ there exists no cut disjoint from $Q_i$ that separates $s_i$ from $t_i$, but does not separate  $s_j$ from $t_j$ for any $j < i$.
There exists a connective list of subgraphs such that every edge of $G$ appears in at most $2\log |V(F)|$ $Q_i$'s.
\end{lemma}
\begin{proof}
We proof this lemma by an induction on $|E(F)|$. 
The base case is when $|E(F)| \leq 2$ for which the proof is trivial.
Now we assume the hypothesis of the induction holds for all forests $F$ such that $|E(F)| < n$ and we prove it for the case of $|E(F)| = n$.\\
If the forest is not connected, then by the hypothesis of the induction, the lemma holds for each connected component and hence it holds for the whole forest. Therefore, without loss of generality, we assume $F$ is a tree. According to Lemma \ref{aux} we can decompose $F$ into two trees $T_1$ and $T_2$ sharing a single vertex and no edges. Now we create two separate lists $L_1$ and $L_2$ in the following way: We start from $i = 1$ and iterate through all pairs of $L$. For each pair $(s_i, t_i)$ we do the following
\begin{enumerate}
	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we add pair $(s_i, t_i)$ to $L_1$.
	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we add pair $(s_i, t_i)$ to $L_2$.
	\item Otherwise, without loss of generality we assume $s_i \in V(T_1)$ and $t_i \in V(T_2)$ and do the following
	\begin{enumerate}
	\item If $(s_i,t_i)$ is the first of such pairs, we do nothing.
	\item If $(s_i,t_i)$ is not the first pair of this type, we add pair $(s_i,s_x)$ to $L_1$ and $(t_i,t_x)$ to $L_2$ where $(s_x,t_x)$ is the first pair with this condition.
	\end{enumerate}
\end{enumerate}

Now, by the hypothesis of the induction we can find connective subgraphs $Q^1 = \langle Q^1_1, Q^1_2, \ldots, Q^1_{|L_1|} \rangle$ and $Q^2 = \langle Q^2_1, Q^2_2, \ldots, Q^2_{|L_2|} \rangle$ for instances of the problem $\langle G, T_1, L_1\rangle$ and $\langle G, T_2, L_2\rangle$ meeting the constraints of the lemma. Next, we create a list of connective subgraphs $Q$ for $\langle G, F, L\rangle$ as follows. For every pair $(s_i, t_i) \in L$ we do the following:
\begin{enumerate}
	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^1$.
	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^2$.
	\item If not both of $s_i$ and $t_i$ are in one of the trees:
	\begin{enumerate}
		\item If $s_i$ and $t_i$ are the first of such pairs, we set $Q_i$ to be the union of the edges in the path from $s_i$ to $t_i$ .
		\item Otherwise let $(s_i,s_x)$ and $(t_i,t_x)$ be the pairs in $L_1$ and $L_2$ associated to $(s_i,t_i)$. We set $Q_i$ to be the union of the subgraphs corresponding $(s_i,s_x)$ and $(t_i,t_x)$ in $Q^1$ and $Q^2$.
	\end{enumerate}
\end{enumerate}
Note that, by the hypothesis of induction every edge appears in no more than $2 \log (\lceil \frac{2}{3} |V(F)|\rceil + 1) \leq 2 \log n - 1$ sets of $Q_1$ and $Q_2$. Apart from the edges of $Q_1$ and $Q_2$, the only new edges in $Q$ are the ones in the path from $s_x$ to $t_x$ that goes through every edge at most once. Therefore, every edge of the graph appears in at most $2 \log n $ subgraphs of $Q$. In the rest we argue that $Q$ is a connective list of subgraphs for $\langle G, F, L\rangle$.

Note that the conditions of the lemma hold for all pairs of vertices $(s_i, t_i)$ that completely lie in one of the trees. Moreover, for the first $(s_x, t_x)$ that is separated by the trees, the conditions are also satisfied since $Q_i$ is a path from $s_x$ to $t_x$ and therefore no disjoint cut from $Q_i$ can separate $s_x$ from $t_x$. All that remains is to show the same properties for the rest of such pairs.  Let $(s_i, t_i)$ be a pair which is separated by the trees and $i > x$. If a cut $c$ disjoint from $Q_i$ separates $s_i$ from $t_i$ and not $s_x$ from $t_x$, then either of $s_i$ or $t_i$ should be separated from both $s_x$ and $t_x$. However, this leads to contradiction because this is guaranteed to not happen due to our construction of $Q_i$ and the fact that both $Q^1$ and $Q^2$ are connective list of subgraphs for $\langle G, T_1, L_1\rangle$ and $\langle G, T_2, L_2\rangle$.
\end{proof}

==> 2nd_proof_useless/log4.tex <==
%In this section we present a poly-logarithmic competitive ratio algorithm for the online weighted degree-bounded Steiner forest problem. To do this, we solve \eqref{LP:sf} with an $O(log^3(n))$ violation on the degree constraints and an $O(log^2(n))$ violation on the weight constraint. Our method uses a similar approach proposed in XX-Debmalia. However applying the same approach results in an $O(log^3(n))$ competitive ratio for both the degree constraints and the weight constraint. Note that we later loose a multiplicative factor of $O(log(n))$ because of lemma XXX. As shown in this section the method in XX-Debmalia can be improved in order to save a factor of $O(log(n))$ on the weight constraint. This improvement makes the competitive ratio of our algorithm $\langle O(log^3(n), O(log^4(n)) \rangle$ for weight and degree bound, respectively.

Let $R$ denote the sequence of requests. For every request $(s_i, t_i)\in R$ we define a collection $\mathcal{S}_i$ of the subsets of $V$. This collection contains every $S\subseteq V$ if and only if $S$ separates $s_i$ from $t_i$ and $S$ has either both or none of $s_j$ and $t_j$ for every $j<i$.

By the definition, $w(opt)$ is the minimum weight of a solution satisfying all degree bound constraints. Therefore, the optimal solution to \ref{LP:sf} is $1$.

\begin{align*}
\text{minimize}           &\quad \quad \alpha \tag{{$\mathbb{LP}1$}}\label{LP:sf}\\
\forall v \in V &\quad\quad  \frac{1}{b_v}\sum_{i\leq |R|}^{}\sum_{e \in \delta(v)}{x_e^i} \leq \alpha\\
&\quad\quad \frac{1}{w(opt)}\sum_{i\leq |R|}^{}\sum_{e \in E}w(e)x_e^i \leq \alpha \\
\forall i \leq |R|, S \in \mathcal{S}_i &\quad\quad \sum_{e \in \delta(S)} {x_e^i} \geq 1 \\
&\quad\quad \x, \alpha \geq 0
\end{align*}

\begin{corollary} \label{opt=1}
	Let $\alpha_{opt}$ be the optimal solution to \eqref{LP:sf}. $\alpha_{opt}=1$.
\end{corollary}

All packing constraints can be written before the arrival of the first request. When a new request $i$ comes, we have to increase $\x$ such that the set of constraint of type $\sum_{e \in \delta(S)} {x_e^i} \geq 1$ are covered for every $S\in \mathcal{S}_i$. To simplify the online scenario, assume that these covering constraints are coming one by one, and we have to satisfy every constraint before the arrival of the next constraint.

Let $m=n+1$ be the number of packing constraints and $d=|E|.|R|$ be the number of variables in $\x$. Define $\mu=1+\frac{1}{3\ln(em)}$ and $\sigma = e^2 \ln(\mu d max\{w(e)\})$. Note that if the maximum weight in $G$ is a polynomial of $n$ then $\sigma \in O(log(n))$. We divide every coefficient in the packing constraints by $2\sigma$. Based on Corollary \ref{opt=1} the optimal of the new LP \eqref{LP_scaled_primal} is $\frac{1}{2\sigma}$. We use the primal-dual technique to find a solution of at most $3\ln(em)$ for the scaled LP. Lemma \ref{lm:main} shows our result is $O(log^2(n))$ competitive.

\noindent
%\begin{minipage}{.44\textwidth} %
	\begin{align}
\text{minimize}  &\quad \alpha \tag{{$\mathbb{P}$}}\label{LP_scaled_primal}\\ \label{deg_bound_constraint}
\forall v \in V &\quad  \frac{1}{2\sigma}\frac{1}{b_v}\sum_{i=1}^{|R|}\sum_{e \in \delta(v)}{x_e^i} \leq \alpha\\ \label{weight_bound_constraint}
&\quad \frac{1}{2\sigma}\frac{1}{w(opt)}\sum_{i=1}^{|R|}\sum_{e \in E}w(e)x_e^i \leq \alpha \\
\forall i \leq |R|, S \in \mathcal{S}_i &\quad \sum_{e \in \delta(S)} {x_e^i} \geq 1 \\ \nonumber
&\quad \x, \alpha \geq 0 \nonumber
	\end{align}
%\end{minipage} %
%\hspace{0.02\textwidth}
%\begin{minipage}{.53\textwidth} %
	\begin{align}
	\text{maximize} &\quad  \sum_{i=1}^{|R|}\sum_{S\in \mathcal{S}_i}{y_{S}^{i}} \tag{{$\mathbb{D}$}}\label{LP_scaled_dual}\\ \label{ineq:dual1}
	\forall e=(u,v), i\leq |R| &\quad \sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \frac{z_u}{2\sigma b_u}+\frac{z_v}{2\sigma b_v}+\frac{w(e) z_w}{2\sigma w(opt)}\\ \label{ineq:dual2}
	&\quad  z_w + \sum_{v=1}^{n}{z_v} \leq 1 \\
	&\quad  z_w, \z_v, y_{S}^{i}\in \mathbb{R}_{\geq 0}
	\end{align}
%\end{minipage}

In the dual LP \ref{LP_scaled_dual} every variable $z_1,\ldots,z_n$ and $z_w$ corresponds to one of the constraints in \ref{deg_bound_constraint} and \ref{weight_bound_constraint} respectively. In our proofs we use $z_w$ and $z_{n+1}$ interchangeably. A dual variable $y_{S}^{i}$ is corresponding to a covering constraint defined by $S\in\mathcal{S}_i$ of request $i$.

For a given vector of variables $\x$ and $1\leq k \leq m$, let $\alpha_k(\x)$ be value of the left hand side of packing constraint $k$, where $\alpha_{n+1}(\x)$ corresponds to \eqref{weight_bound_constraint}. Let $\alpha(\x)=\max_{1\leq k\leq m}\{\alpha_k(\x)\}$. Our goal is to find a feasible $\x$ that minimizes $\alpha(\x)$.

The potential function $\Phi(\x)$ is defined as follows
 $$\Phi(\x) := \ln\big( \sum_{k=1}^{m}\exp(\alpha_k(\x)) \big) \enspace .$$
Since $\alpha(\x)\leq \Phi(\x) \leq \alpha(\x)+\ln(m)$, we use this potential function as an estimate of $\alpha(\x)$.

% make sure that the modification you made does not hurt the whole proof

The algorithm initializes the variables with a vector $\x^0$ with $1/(d \max_{e\in E}\{w(e)\})$ for each variable $x_{e}^{i}$, $e\in E$ and $1\leq i\leq |R|$.

\begin{lemma}
	$\Phi(\x^0) \leq 1/(2\sigma) + \ln(m)$.
\end{lemma}
\begin{proof}
	For every packing constraint $1 \leq v \leq n$:
	$$\alpha_v(\x^0) \leq d \frac{1}{d\max_{e\in E}\{w(e)\}} \frac{1}{2\sigma b_v}\leq \frac{1}{2\sigma} \enspace .$$
	For constraint $n+1$:
	$$\alpha_{n+1}(\x^0) \leq d \frac{1}{d\max_{e\in E}\{w(e)\}}\frac{\max_{e\in E}\{w(e)\}}{2\sigma w(opt)} \leq \frac{1}{2\sigma} \enspace .$$
	Hence,
	$$\Phi(\x^0) = \ln\big( \sum_{k=1}^{n+1}\exp(\alpha_k(\x^0)) \big) \leq \ln\big(\sum_{k=1}^{m}\exp(1/(2\sigma))\big) \leq \frac{1}{2\sigma} + \ln(m) \enspace .$$
\end{proof}

To satisfy a new covering constraint we do multiplicative updates on every variable. For every $e=(u,v)\in E$ and $1\leq i\leq |R|$, define
\begin{align*}
	rate_{e,i}(\x) = \frac{\partial \Phi(\x)}{\partial x_{e}^{i}}&=\frac{e^{\alpha_u(\x)}/(2\sigma b_u)+e^{\alpha_v(\x)}/(2\sigma b_v)+e^{\alpha_w(\x)}w(e)/(2\sigma w(opt))}{ \sum_{k=1}^{m}e^{\alpha_k(\x)}} \\
	&= \frac{e^{\alpha_u(\x)}/b_u+e^{\alpha_v(\x)}/b_v+e^{\alpha_w(\x)}w(e)/w(opt)}{ 2\sigma\sum_{k=1}^{m}e^{\alpha_k(\x)}} \enspace .
\end{align*}

For a covering constraint corresponding to $S\in \mathcal{S}_i$ of request $i$, define
$$\epsilon_{S}^{i}(\x) = (\mu-1)\min_{e\in\delta(S)}\{rate_{e,i}(\x)\}$$
so that for all $e \in \delta(S)$, $\epsilon_{S}^{i}(\x) / rate_{e,i}(\x) \leq \mu-1$. For this covering constraint there is a variable $y_{S}^{i}$ in the dual LP \eqref{LP_scaled_dual}. Repeat the following steps until the constraint is satisfied ($\sum_{e \in \delta(S)} {x_e^i} \geq 1$).
\begin{itemize}
\item Let $\x^l$ be the current value of variables in \eqref{LP_scaled_primal}.
\item For each $e\in \delta(S)$, multiply $x_{e}^{i}$ by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$.
\item Add $e\epsilon_{S}^{i}(\x^l)$ to dual variable $y_{S}^{i}$.
\end{itemize}

A single iteration of the above loop is called a \textit{phase} indexed by $l$. Let $L_{S}^{i}$ be the set of all phases executed for constraint $S\in\mathcal{S}_i$ of request $i$, and $L=\cup L_{S}^{i}$. Note that in every phase variables are multiplied by a factor of at most $\mu$.

\begin{lemma}
	\label{rate_ratio}
	For a given $\x$ and $\x'$ with $\alpha(\x)\leq 3\ln(m)$, if $x_{e}^{i} \leq x_{e}^{\prime i} \leq \mu x_{e}^{i}$ for every $1\leq i \leq |R|$ and $e\in E$, then
	$$rate_{e, i}(\x') \leq e \, \text{rate}_{e, i}(\x) \enspace .$$
\end{lemma}

\begin{proof}
	Since $\alpha_k(\x)\leq \alpha(\x) \leq 3\ln(em)$,
	\begin{align*}
		\mu \alpha_k(\x)
		\leq \bigg(1+\frac{1}{3\ln(em)}\bigg)\alpha_k(\x)
		\leq \alpha_k(\x)+\frac{\alpha_k(\x)}{3\ln(em)}
		\leq \alpha_k(\x)+\frac{\alpha(\x)}{3\ln(em)}
		\leq \alpha_k(\x)+1 \enspace .
	\end{align*}
	By the linearity of constraints,
	\begin{align}
		\label{ineq1}
		\forall k: \quad\quad \alpha_k(\x) \leq \alpha_k(\x') \leq 	\mu \alpha_k(\x)  \leq \alpha_k(\x)+1 \enspace .
	\end{align}
	Using \ref{ineq1} in the definition of $rate_{e,i}(\x')$,
	\begin{align*}
	rate_{e,i}(\x')&= \frac{e^{\alpha_u(\x')}/b_u+e^{\alpha_v(\x')}/b_v+e^{\alpha_w(\x')}w(e)/w(opt)}{ 2\sigma\sum_{k=1}^{m}e^{\alpha_k(\x')}}
	 \\
	&\leq
	\frac{e^{\alpha_u(\x)+1}/b_u+e^{\alpha_v(\x)+1}/b_v+e^{\alpha_w(\x+1)}w(e)/w(opt)}{ 2\sigma\sum_{k=1}^{m}e^{\alpha_k(\x+1)}} \\
	&= e \bigg ( \frac{e^{\alpha_u(\x)}/b_u+e^{\alpha_v(\x)}/b_v+e^{\alpha_w(\x)}w(e)/w(opt)}{ 2\sigma\sum_{k=1}^{m}e^{\alpha_k(\x)}}
	 \bigg ) \\
	&= e \, rate_{e, i}(\x) \enspace .
	\end{align*}
\end{proof}

\begin{lemma}
	The increase in $\sum_{i=1}^{|R|}\sum_{S\in \mathcal{S}_i}{y_{S}^{i}}$ is an upper bound for the total increase in $\Phi(\x)$.
\end{lemma}

\begin{proof}
	To prove the lemma we show that in every phase $l$ the amount of increase in the potential function, $\Phi(\x^{l+1})-\Phi(\x^l)$, is at most the amount of increase in the corresponding dual variable $y_{S}^{i}$. Suppose that at this phase $l$, the algorithm is trying to satisfy a covering constraint $S\in\mathcal{S}_i$of request $1\leq i\leq |R|$. We show that the amount of increase in the potential function is at most $e\epsilon_{S}^{i}(\x^l)$.
	
	Let $\x(t):=\x^l + (\x^{l+1}-\x^l)t$ for $0\leq t\leq 1$. Base on this function, we define $\phi(t):=\Phi(\x(t))$ and $rate_{e,i}(t):=rate_{e,i}(\x(t))$. The derivative of $\phi(t)$ is 
	\begin{align}
		\frac{\partial \phi(t)}{\partial t} = \sum_{e\in \delta(S)} \frac{\partial \phi(t)}{\partial x_{e}^{i}(t)}\frac{\partial x_{e}^{i}(t)}{\partial t} = \sum_{e\in\delta(S)} rate_{e,i}(t)\frac{\partial x_{e}^{i}(t)}{\partial t} \enspace .
	\end{align}
	From lemma \ref{rate_ratio} we have $rate_{e,i}(t)\leq e\, rate_{e,i}(0)=e \, rate_{e,i}(\x^l)$. Therefore,
	\begin{align}
		\nonumber
		\Phi(\x^{l+1})-\Phi(\x^l) &= \int_{0}^{1} \frac{\partial \phi(t)}{\partial t} dt \\ \nonumber
		&= \int_{0}^{1} \sum_{e\in \delta(S)} rate_{e,i}(t)\frac{\partial x_{e}^{i}(t)}{\partial t} dt\\ \nonumber
		&\leq e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\int_{0}^{1} \frac{\partial x_{e}^{i}(t)}{\partial t} dt\\ \nonumber
		&=  e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i}(1)-x_{e}^{i}(0)\big) \\ \label{diff_x}
		&=  e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i,l+1}-x_{e}^{i,l}\big) \enspace .
	\end{align}
	Recall that in phase $l$ we multiply $x_{e}^{i}$ by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$  for every $e\in\delta(S)$. Hence, the difference between $x_{e}^{i,l+1}$ and $x_{e}^{i,l}$ in \eqref{diff_x} is exactly $x_{e}^{i,l}\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$.
	\begin{align}
		\nonumber
		\Phi(\x^{l+1})-\Phi(\x^l) &\leq e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i,l+1}-x_{e}^{i,l}\big) \\ \nonumber
		&= e\,\epsilon_{S}^{i}(\x^l)\sum_{e\in\delta(S)}x_{e}^{i,l}\\
		&\leq e\,\epsilon_{S}^{i}(\x^l) \enspace .
	\end{align}
	The last inequality holds because the covering constraint is not satisfied before the execution of phase $l$.
\end{proof}

\begin{lemma}
	For every $e\in E$ and $1\leq i\leq |R|$,
	$$\sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \sigma \max_{l\in L}\{rate_{e,i}(x^l)\} \enspace .$$
\end{lemma}

\begin{proof}
	In every phase $l$, $x_{e}^{i}$ is multiplied by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l) \geq \exp\bigg(\frac{\epsilon_{S}^{i}(\x^l)}{e\,rate_{e,i}(\x^l)}\bigg)$, where the inequality comes from $1+a\geq\exp(a/e)$ for $0\leq a\leq 1$. Moreover, the initial value of $x_{e}^{i}$ is $1/(d\max_{e\in E}\{w(e)\})$ and will never exceed $\mu$, because otherwise $x_{e}^{i}$ satisfies the phase termination condition.
	$$
	\frac{1}{d\max_{e\in E}\{w(e)\}}\prod_{S\in\mathcal{S}_i:e\in\delta(S)}\prod_{l\in L_{S}^{i}}\exp\bigg(\frac{\epsilon_{S}^{i}(\x^l)}{e\,rate_{e,i}(\x^l)}\bigg) \leq x_{e}^{i} \leq \mu \enspace .
	$$
	By multiplying both sides by $d\max_{e\in E}\{w(e)\}$ and taking natural log, 
	$$
	\label{ineq:vasati}
	\sum_{S\in\mathcal{S}_i:e\in\delta(S)}\sum_{l\in L_{S}^{i}}\frac{{\epsilon_{S}^{i}(\x^l)}}{e\,rate_{e,i}(\x^l)}
	\leq \ln\big(\mu d \max_{e\in E}\{w(e)\}\big ) \enspace .
	$$
	By multiplying both sides by $e\,\max_{l\in L}\{rate_{e,i}(\x^l)\}$ we get
	\begin{align}
		\label{ineq:sakhte}
		\sum_{S\in\mathcal{S}_i:e\in\delta(S)}\sum_{l\in L_{S}^{i}}{\epsilon_{S}^{i}(\x^l)} \leq e\,\ln\big(\mu d \max_{e\in E}\{w(e)\}\big) \max_{l\in L}\{rate_{e,i}(\x^l)\} \enspace .
	\end{align}	
	From the updates of the algorithm, a dual variable $y_{S}^{i}$ is exactly $e\sum_{l\in L_{S}^{i}}\epsilon_{S}^{i}(\x^l)$. On the other hand $\sigma\geq	e^2\,\ln(\mu d \max_{l\in L}\{rate_{e,i}(\x^l)\})$, therefore by multiplying both sides of Inequality \ref{ineq:sakhte} by $e$ we have
	\begin{align}
	\label{ineq:sakhe_final}
	\sum_{S\in\mathcal{S}_i:e\in\delta(S)}y_{S}^{i} \leq \sigma \max_{l\in L}\{rate_{e,i}(\x^l)\} \enspace .
	\end{align}
\end{proof}


Now we set dual variables $z_k$ so that for every $e=(u,v)\in E$ and $1\leq i \leq |R|$ the right hand side of \eqref{ineq:dual1}  is at least $\max_{l\in L}\{rate_{e,i}(\x^l)\}$. This makes every constraint in \eqref{ineq:dual1} being violated by a factor of at most $\sigma$.

By the definition,

\begin{align*}
	\max_{l\in L}\{rate_{e,i}(\x^l)\} &= \max_{l\in L}\bigg\{\frac{e^{\alpha_u(\x^l)}/b_u+e^{\alpha_v(\x^l)}/b_v+w(e)e^{\alpha_w(\x^l)}/w(opt)}{\sigma \sum_{k=1}^{m}e^{\alpha_k(\x^l)}}\bigg\} \\
	&\leq \frac{1}{\sigma b_u}\max_{l\in L}\bigg\{\frac{e^{\alpha_u(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} +
	\frac{1}{\sigma b_v}\max_{l\in L}\bigg\{\frac{e^{\alpha_v(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} +
	\frac{w(e)}{\sigma w(opt)}\max_{l\in L}\bigg\{\frac{e^{\alpha_w(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} \enspace .
\end{align*}

Therefore, setting $z_k=\max_{l\in L}\bigg\{\frac{\exp(\alpha_k(\x^l))}{\sum_{k'=1}^{m}\exp(\alpha_{k'}(\x^l))}\bigg\}$ for every $k$ attains our goal.
	
\begin{corollary} \label{cor:dual_violation}
	For every $e=(u,v)\in E$ and $1\leq i\leq |R|$,
	$$ \sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \sigma\bigg(\frac{z_u}{2\sigma b_u}+\frac{z_v}{2\sigma b_v}+\frac{w(e) z_w}{2\sigma w(opt)}\bigg) \enspace .$$
\end{corollary}

In the following lemma, we find an upper bound for the left hand side of \eqref{ineq:dual2}. In Lemma \ref{lm:main} use this upper bound to construct a solution for the dual LP.

\begin{lemma} \label{lm:dual_ineq2}

		$\label{ineq:dual_ineq2}
		\sum_{k=1}^{m} z_k \leq \ln(em) + \max_{l\in L}\{\alpha(\x^l)\} \enspace .$
\end{lemma}

\begin{proof}
	For each packing constraint $k$, define
	$$\ind(k) := \argmax_{l\in L}\bigg\{\frac{e^{\alpha_k(\x^l)}}{\sum_{k'=1}^{m}e^{\alpha_{k'}(\x^l)}}\bigg\} \enspace .$$
	Thus $\ind(k)$ is the phase in which $z_k$ attains its value. Without loss of generality, we reorder the packing constraints in \ref{LP_scaled_primal} such that $\ind(l)<\ind(k)$ for every $l<k$. We use the following bound in order to prove the lemma.
	\begin{lemma} [Azar et al. \cite{XXX}] \label{lm:azar_khanum}
		For $m\in \mathbb{Z}_{+}$ and $a_1,\ldots,a_m \in \mathbb{R}_{\geq 0}$ with $a_1>0$, $$\sum_{i=1}^{m}\frac{a_i}{\sum_{j\leq i}a_j} \leq 1 + \ln\bigg (\frac{\sum_{i=1}^{m}a_i}{a_1} \bigg) \enspace . $$
	\end{lemma}
	
	Let $a_k:=\exp(\alpha_k(\x^{\ind(k)}))$. Since the primal variables are non-decreasing in time, $\alpha_l(x^{\ind(k)})\geq \alpha_l(x^{\ind(l)})$. Therefore for every $k$,
	\begin{align}
		\label{ineq:zkak}
		z_k &= \frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{m}\exp(\alpha_{l}(\x^{\ind(k)}))}
		\leq \frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{k}\exp(\alpha_{l}(\x^{\ind(k)}))}
		\leq
		\frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{k}\exp(\alpha_{l}(\x^{\ind(l)}))}
		=\frac{a_k}{\sum_{l\leq k}a_l} \enspace .
	\end{align}
	From Inequality \eqref{ineq:zkak} and Lemma \ref{lm:azar_khanum} we have
	\begin{align} \label{ineq:p1}
		\sum_{k=1}^{m}z_k\leq \sum_{k=1}^{m}\frac{a_k}{\sum_{l\leq k}a_l} \leq 1 + \ln\bigg (\frac{\sum_{k=1}^{m}a_k}{a_1} \bigg) \enspace .
	\end{align}
	Considering the fact that $\alpha_1(\x^{\ind(1)})\geq 0$, and $a_1\geq 1$,
	\begin{align} \label{ineq:p2}
		1 + \ln\bigg (\frac{\sum_{k=1}^{m}a_k}{a_1} \bigg) \leq 1 + \ln\big (\sum_{k=1}^{m}a_k\big) \leq 1 + \ln(m) + \ln\big(\max_{k}(a_k)\big) \enspace .
	\end{align}
	By the definition of $a_k$,
	\begin{align} \label{ineq:p3}
		1 + \ln(m) + \ln\big(\max_{k}(a_k)\big) \leq \ln(em) + \ln\big(\max_{l}\big(\exp(\alpha(\x^l))\big)\big) \leq \ln(em) + \max_{l\in L}(\alpha(\x^l)) \enspace .
	\end{align}
 	The proof follows from the Inequalities \eqref{ineq:p1}, \eqref{ineq:p2}, and \eqref{ineq:p3}.
\end{proof}

%Using Corollary \ref{cor:dual_violation} and Lemma \ref{lm:dual_ineq2} we make a feasible solution dual LP \ref{LP_scaled_dual}.

Using the previous lemmas we can now prove an upper bound on the competitive ratio of the algorithm.

\begin{lemma} \label{lm:main}
	The algorithm is $6\sigma\ln(em)$-competitive.
\end{lemma}

\begin{proof}
	Define $\nu:=\ln(em)+\alpha(\x^l)$. The dual problem is a maximization problem, and Corollary \ref{cor:dual_violation} and Lemma \ref{lm:dual_ineq2} show that $\z/\nu$ and $\y/(\sigma\nu)$ are feasible values for the dual variables. By weak duality, any feasible dual solution is a lower bound on the optimal primal solution, and hence $\sum_{i=1}^{|R|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}/(\sigma\nu)\leq \frac{1}{2\sigma}$. Note that the optimum of scaled primal  \ref{LP_scaled_primal} is $\OPT=\frac{1}{2\sigma}$.
	The dual objective $\sum_{i=1}^{|R|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}$ is an upper bound on the total increase in $\Phi(\x)$. At the beginning, $\Phi(\x^0)\leq \frac{1}{2\sigma}+\ln(m)$. $\Phi(\x)$ is itself an upper bound for $\alpha(\x)$. Therefore,
	\begin{align} \label{ineq:upperbound}
		\alpha(\x)\leq \frac{1}{2\sigma}+\ln(m)+\sum_{i=1}^{|R|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}\leq \frac{1}{2\sigma}+\ln(m)+\frac{\nu}{2} \enspace .
	\end{align}
	
	Substituting $\nu=\ln(em)+\alpha(\x)$ yields $\alpha(\x)\leq 3\ln(em)$, and $\nu=\ln(em)+\alpha(\x)\leq 4\ln(em)$. Considering $\OPT=\frac{1}{2\sigma}$ and plugging in the upper bound of $\nu$ in Inequality \eqref{ineq:upperbound} the competitive ratio of the algorithm is obtained.
	
	\begin{align*}
		\alpha(\x) &\leq \frac{1}{2\sigma}+\ln(m)+\frac{\nu}{2} \\
		&\leq \OPT + 2\sigma\ln(m) \OPT + 4\sigma\ln(em)\OPT \\
		&\leq 6\sigma\ln(em)\OPT \enspace .
	\end{align*}
\end{proof}




==> 2nd_proof_useless/preliminaries.tex <==
Let $G=(V, E)$ be an undirected graph with $n$ vertices and $m$ edges. Let $w:E \rightarrow \mathbb{R}_{>0}$ be a function denoting the edge weights. For every vertex $v \in V$ let $b_v \in \mathbb{Z}_{>0}$ denote the degree bound of $v$. Let $\deg_H(v)$ denote the degree of vertex $v$ in subgraph $H \subseteq G$. We define load of vertex $v$ w.r.t. $H$ as $\deg_H(v)/b_v$. In \dbsf{} we are given graph $G$, degree bounds, and $k$ connectivity demands. The $i$-th demand is a pair of vertices $(s_i, t_i)$, where $s_i, t_i \in V$. In \dbsf{} the goal is to find a subgraph $H \subseteq G$ such that for each demand $i$, $s_i$ is connected to $t_i$ in $H$, for each vertex $v \in V$, $l_H(v) \leq 1$, and total weight of $H$ ($\sum_{e\in E(H)}w(e)$) is minimized. Let $opt$ denote an optimal solution. In this paper without loss of generality we assume the demand endpoints are distinct vertices with degree one in $G$ and degree bound infinity.

In online variant of the problem, we are given graph $G$ and degree bounds in advance. However the sequence of demands are given one by one. At arrival of demand $i$, we are asked to provide a subgraph $H_i$, such that $H_{i-1} \subseteq H_i$ and $s_i$ is connected to $t_i$ in $H_i$.

We formalize the problem as online mixed packing and covering programs. The following is a general mixed packing and covering IP, where $P$ and $C$ are a set of packing and covering constraints, respectively. For example the $i$-th packing constraint is $\sum_j{p_{ij}x_j}\leq \alpha$.

\begin{align*}
\text{minimize}           &\quad \alpha \tag{{$\mathbb{IP}1$}}\label{IP:pc}\\
&\quad\quad  P\x \leq \alpha\\
&\quad\quad C\x \geq 1 \\
&\quad\quad \x, \alpha \in \mathbb{Z}_{>0}
\end{align*}

In online variant of mixed packing and covering IP, we are given the packing constraints in advance. However the covering constraints arrive in an online manner. At arrival of each covering constraint we should update the solution $\x$ such that it satisfies the new covering constraint as well as the previous ones. Moreover the previous decisions cannot be changed. In other words, we can only increase $\x$.


For now I bring the following two LPs such that everyone can refer to the same LP. However we have to define the modified problem in which you have to buy a new path to one of previous terminals (In tree version. In forest version it is more complicated). We should mention that the following LPs are for that problem.

Let $\mathcal{S}$.

\begin{align*}
\text{minimize}           &\quad \alpha \tag{{$\mathbb{LP}1$}}\label{LP:sf}\\
\forall v \in V &\quad\quad  \frac{1}{b_v}\sum_{i}^{}\sum_{e \in \delta(v)}{x_e^i} \leq \alpha\\
\forall t_i,S \text{ separating } t_i \text{ and } t_1, \ldots, t_{i-1}             &\quad\quad \sum_{e \in \delta(S)} {x_e^i} \geq 1 \\
&\quad\quad \frac{1}{w(opt)}\sum_i\sum_{e \in E}w(e)x_e^i \leq \alpha \\
&\quad\quad \x, \alpha \geq 0
\end{align*}

\begin{align*}
\text{minimize}           &\quad \alpha \tag{{$\mathbb{IP}2$}}\label{IP:sf}\\
\forall v \in V &\quad\quad  \frac{1}{b_v}\sum_{H \subseteq G}{\deg_H(v)x_H} \leq \alpha\\
\forall t_i            &\quad\quad \sum_{H\text{ satisfies connectivity }} {x_H} \geq 1 \\
&\quad\quad \frac{1}{w(opt)}\sum_{H\subseteq G}w(H)x_H \leq \alpha \\
&\quad\quad \x, \alpha \geq 0
\end{align*}

==> OMPC.tex <==
	In this section we consider a class of online mixed packing and covering integer programs which have specific covering constraints. We provide an online algorithm that violates each packing constraint by at most a factor of $O(\log |P|)$, where $|P|$ is the number of packing constraints. We note that this bound is independent of the number of variables, the number of covering constraints, and the coefficients. Moreover the algorithm is for integer programs, which implies there is no need for (online) rounding.
	
	In particular we prove any online mixed packing and covering IP has an online solution of $O(\log|P|)$ if it satisfies the following properties:
	\begin{itemize}
		\item[(I)]\label{c:1} Each variable $x_k \in \{0, 1\}$. 
		\item[(II)]\label{c:2} Every variable has non-zero coefficient in exactly one covering constraint.
		%\item[(II)]\label{c:2} For each covering constraint, every coefficient is either zero or one.
	\end{itemize}
	
	The algorithm is as follows. Initially we assume the optimal solution is one. Whenever the algorithm fails to find a feasible solution with $\alpha=1$, we do the failure stage, which is: (i) divide every coefficient in packing constraints by two, (ii) ignore previous values of $\x$, and (iii) start adding covering constraints from the beginning in the new IP. We initially set $\x=0$. At arrival of $j+1$-th covering constraint, do the following. Let $S=\{x_{s_1}, x_{s_2}, \ldots, x_{s_{|S|}}\}$ be a subset of variables. Let $C_{j+1}(x_{s_k})$ denote the coefficient of $x_{s_k}$ in the $j+1$-th covering constraint. Let $P_i$ be the $i$-th packing constraint and $P_{ik}$ denote the coefficient of $x_k$ in $i$-th packing constraint. For each packing constraint $P_i$, let $v_{P_i}(S):=\sum_{k=1}^{|S|}P_{is_k}$. We say $S$ satisfies $j+1$-th constraint if it has the following properties.
	\begin{itemize}
		\item $\sum_{k=1}^{|S|}C_{j+1}(x_{s_k}) \geq 1$.
		\item For each packing constraint $i$, $v_{P_i}(S) \leq 1$. In other words setting all variables in $S$ equal to one, does not violate any packing constraint by itself.
	\end{itemize}
	Furthermore, for each set $S$ we define a cost function
	 $\tau_{S}(j):=\sum_{i=1}^{|P|}\rho^{P_{i}\cdot\x(j)+v_{P_i}(S)}-\rho^{P_i\cdot\x(j)}$, where $\rho>1$ is a constant to be defined. Now we choose a set $S$ such that $S$ satisfies $j+1$-th constraint and $\tau_{S}(j)$ is minimized. We set each variable $x_{s_k}$ in $S$ equal to one. If there is no such $S$, we do the failure stage.
	 %Then we choose the variable $x_l$ that can satisfy covering constraint $j+1$ and has the minimum cost. Note that by Condition (II), setting each variable to one either makes no change on $j+1$-th covering constraint or satisfies it completely.
	
		\begin{algorithm}[!h]
			\textbf{Input:} Packing constraints $P$, and an online stream of covering constraints $C_1, C_2, \ldots$.
			
			\textbf{Output:} A feasible solution for OMPC such that every given covering constraint is satisfied; Or failure.
			
			%		\textbf{Offline Process:}
			%		\begin{algorithmic}[1]
			%			\STATE Initialize $H=\varnothing$.
			%		\end{algorithmic}
			
			\textbf{Online Scheme; assuming a covering constraint $C_{j+1}$ is arrived:}
			
			\begin{algorithmic}[1]
				\STATE $S \gets \argmin_{S \subseteq \{x_1, \ldots, x_n\}}\{\tau_S(j)\ |\ S \text{ satisfies } C+1\text{-th covering constraint}\}$.
				\IF{$S = \emptyset$}
					\STATE return failure.
				\ENDIF
				\FORALL {$x_k \in S$}
				\STATE $x_k \gets 1$.
				\ENDFOR
			\end{algorithmic}
			\caption{To be defined}
			\label{alg:OMPC}
		\end{algorithm}

	Now we prove Algorithm \ref{alg:OMPC} has competitive ratio $O(\log|P|)$. The general proof idea is as follows. First we assume the optimal offline solution of the integer program is one. which means there is an optimal solution that does not violate any packing constraint. Afterwards we define a potential function for each online stage of the algorithm. We prove that the potential function is not increasing after satisfying each covering constraint. This can imply the competitive ratio $O(\log|P|)$. Then we can show if the optimal solution is greater than one, we can use a doubling method to update our guess and lose another factor of 4. In particular at each stage if the guess is not right, we divide each packing coefficient by two and ignore the solution so far. The total violation of these solutions is no more than twice the final solution. Since we are guessing $\alpha$ is a power of 2, we lose another factor of 2.
	
	\begin{lemma}
		If the optimal solution of Mixed packing and covering IP is one, Algorithm \ref{alg:OMPC} has competitive ratio $O(\log |P|)$.
	\end{lemma}
	\begin{proof}
		Let $\x(j)$ and $\x^*(j)$ denote the solution of Algorithm \ref{alg:OMPC} and an optimal solution at online stage $j$, respectively. For each online stage $j$, we define a potential function $\Phi_j$ as follows
	\begin{equation}\label{eq:phi}
	\Phi_j=\sum_{i=1}^{|P|} \rho^{P_i\cdot\x(j)} (\gamma - P_i\cdot\x^*(j))\enspace,
	\end{equation}

%	The general idea of the proof is that at each online stage $\Phi$ is non-increasing, which implies for each $j$ $\Phi_j \geq \Phi_0=\gamma m$.

	where $\gamma>1$ is a constant to be defined later. Due to \eqref{eq:phi}:
	\begin{equation}\label{eq:pot}
	\Phi_{j+1}-\Phi_j=\sum_{i=1}^{|P|} \rho^{P_i\cdot\x(j+1)} (\gamma - P_i\cdot\x^*(j+1)) - \rho^{P_i\cdot\x(j)} (\gamma - P_i\cdot\x^*(j))\enspace.
	\end{equation}
	Let $S$ be the set chosen by Algorithm \ref{alg:OMPC} for $j+1$-th covering constraint. By Condition (II) each variable in $j+1$-th covering constraint has zero coefficient in $j$ first covering constraints. Therefore we can assume the optimal solution sets a set of variables $S^*={x_{s^*_1}, \ldots, x_{s^*_{|S^*|}}}$ equal to 1 at this stage. Thus we can write Equation \eqref{eq:pot} as:
	\begin{align}\label{eq:pot2}
	\Phi_{j+1}-\Phi_j=&\sum_{i=1}^{|P|}{(\gamma-P_i\cdot\x^*(j))(\rho^{P_i\cdot\x(j)+v_{P_{i}}(S)} - \rho^{P_i\cdot\x(j)})}-{\rho^{P_i\cdot\x(j+1)}v_{P_i}(S^*)} &\text{Since }P_i\cdot\x^*(j) \geq 0\\\nonumber
	\leq&\sum_{i=1}^{|P|}{\gamma(\rho^{P_i\cdot\x(j)+v_{P_i}(S)} - \rho^{P_i\cdot\x(j)})}-{\rho^{P_i\cdot\x(j+1)}v_{P_i}(S^*)}
	&P_i\cdot\x(j+1) \geq P_i\cdot\x(j)\\\nonumber
	\leq&\sum_{i=1}^{|P|}{\gamma(\rho^{P_i\cdot\x(j)+v_{P_i}(S)} - \rho^{P_i\cdot\x(j)})}-{\rho^{P_i\cdot\x(j)}v_{P_i}(S^*)}\enspace.
	\end{align}
	Now according to the algorithm for each subset $S'=\{x_{s'_1}, x_{s'_2}, \ldots, x_{s'_{|S'|}}\}$ such that $\sum_{k=1}^{|S|}C_{j+1}(x_{s_k})\geq 1$, either $\tau_{S}(j) \leq \tau_{S'}(j)$ or there exists a packing constraint $P_i$ such that $v_{P_i}(S') > 1$. Since for every $P_i$, $v_{P_i}(S^*) \leq 1$, then $\tau_{S}(j) \leq \tau_{S^*}(j)$. Thus $\rho^{P_i\cdot\x(j)+v_{P_i}(S)} - \rho^{P_i\cdot\x(j)} \leq \rho^{P_i\cdot\x(j)+v_{P_i}(S^*)} - \rho^{P_i\cdot\x(j)}$. Therefore we can rewrite Inequality \eqref{eq:pot2} as
	\begin{align}
	\Phi_{j+1}-\Phi_j\leq&\sum_{i=1}^{|P|}{\gamma(\rho^{P_i\cdot\x(j)+v_{P_i}(S^*)} - \rho^{P_i\cdot\x(j)})}-{\rho^{P_i\cdot\x(j)}v_{P_i}(S^*)}
	\\\nonumber
	=&\sum_{i=1}^{|P|}{\rho^{P_i\cdot\x(j)}(\gamma \rho^{v_{P_i}(S^*)}-\gamma-v_{P_i}(S^*))}\enspace.
	\end{align}
	We would like to set $\rho$ and $\gamma$ such that $\Phi_j$ is non-increasing. We set $\rho$ and $\gamma$ such that for each packing constraint $P_i$, $\gamma \rho^{v_{P_i}(S^*)}-\gamma-v_{P_i}(S^*) \leq 0$. Thus
	\begin{align}
	\gamma\rho^{v_{P_i}(S^*)}-\gamma &\leq v_{P_i}(S^*) \quad\quad &\text{Since $0 \leq v_{P_i}(S^*) \leq 1$}\\
	\gamma\rho{v_{P_i}(S^*)}-\gamma &\leq v_{P_i}(S^*)\quad\quad &\text{By simplifying}\\
	\rho &\leq 1+1/\gamma\enspace.
	\end{align}
	
	Thus we can set $\rho$ and $\gamma$ such that $\Phi_j$ is non-increasing. Since $\x(0)=\x^*(0)=0$, $\Phi_0=\gamma |P|$. Thus at each stage $j$, $\Phi_j\leq \Phi_0=\gamma|P|$. Therefore for each constraint $P_i$,
	\begin{align}
	\rho^{P_i\cdot\x(j)}(&\gamma-P_i\cdot\x^*(j)) \leq \gamma|P|\enspace.
	\end{align}
	Thus,
	\begin{align}
	\rho^{P_i\cdot\x(j)} &\leq \frac{\gamma|P|}{(\gamma-P_i\cdot\x^*(j))} \quad\quad &\text{Since $P_i\cdot\x^*(j) \leq 1$}\\
	&\leq \frac{\gamma|P|}{\gamma-1}\enspace.
	\end{align} 
	Thus we can conclude $P_i\cdot\x(j) \in O(\log |P|)$.
	\end{proof}

==> acknowledgement.tex <==
\section{Acknowledgment}
We would like to thank Shi Li for having very helpful discussions and introducing the rounding methods to us.

==> dep_rouding.tex <==
\subsection{Rounding}
In this section we present a rounding method to obtain an integer solution for every optimal solution of LP \ref{lplabel} when the underlying metric is a line. The high-level idea of the method is as follows: We first split the servers into small pieces where every piece has a mass of $\epsilon$ and represents an $\epsilon$ fraction of a server. We assume $\epsilon$ is small enough to make sure the value of all variables in the solution of the LP can be written as the multiplication of $\epsilon$ to an integer number. Next, we show for every optimal solution of the linear program we can associate a path to every fractional server such that (i) The flow of every edge in the LP is equal to the total mass of fractional servers going through that edge (ii) The order of fractional servers is preserved as they move along the edges. Finally we show that an optimal integral solution of the program can be determined by just following a set of $k$ fractional servers.

Similar to equivalence of the integral solutions of LP \ref{lplabel} and online algorithms for the corresponding instance of the stochastic k-server, every fractional solution of LP \ref{lplabel} can be seen as an online fractional algorithm that reports a fractional configuration upon arrival of every request. Now, every fractional configuration is consisted of many fractional  

==> fractional.tex <==
\section{Fractional Solutions}\label{fsf}

In this section we provide a fractional online algorithm for the $k$-server problem that can be implemented in polynomial time. Note that by Theorem \ref{thebest} we know that there exist configurations $\langle \B_1, \B_2, \ldots, \B_t\rangle$ such that the expected cost of a non-adaptive algorithm that always returns these configurations is at most 3. Therefore, we write an integer program to find such configurations with the least expected cost. Next, we provide a relaxed LP of the integer program and show that every feasible solution of such LP corresponds to a fractional online algorithm for the stochastic $k$-server problem. Hence, solving such a linear program, that can be done in polynomial time, gives us a fractional online algorithm for the problem.

%\snote{I should define the graph here.}

\subsection{Linear Program}
 Recall that given $t$ independent distributions $\langle P_1, \ldots, P_t \rangle$ for online stochastic $k$-server, an adaptive algorithm can be represented by $t+1$ configurations $\langle B_0, \ldots, B_t \rangle$. Upon the arrival of each request $r_i$, we move the servers from configuration $B_{i-1}$ to $B_i$ and then one server serves $r_i$ and goes back to its position in $B_i$. The objective is to find the configurations such that the cost of moving to new configurations in addition to the expected cost of serving the requests is minimized. Therefore the problem can formulated in an offline manner. First we provide an integer program in order to find a vector of configurations with the least cost.
 
 The decision variables of the program represent the configurations, the movement of servers from one configuration to another, and the way that each possible request is served. In particular,
 at each time step $\tau$:
 \begin{itemize}
 	\item For each node $v$ there is a variable $b_{\tau, v} \in N$ denoting the number of servers on node $v$. 
 	\item For each pair of nodes $u$ and $v$, there is a movement variable $f_{\tau, u, v} \in N$ denoting the number of servers going from $u$ to $v$ for the next round.
 	\item For each node $v$ and possible request node $r$, there is a variable $x_{\tau, v, r} \in \{0, 1\}$ denoting whether $r$ is served by $v$ or not.
 \end{itemize}
 
 In the following integer program, the first set of constraints ensures the number of servers on nodes at each time is updated correctly according to the movement variables. The second set of constraints ensures that each possible request is served by at least one server. The third set of constraints ensures that no possible request is served by an empty node. By the definition, the cost of a sequence of configurations $\langle B_0, \ldots, B_t \rangle$ is $\sum_{i=1}^t d(B_{i-1}, B_i)+2 \sum_{i=1}^t d(B_i, r_i)$. Thus the objective is to minimize the expression $$\sum_\tau\sum_{u, v}f_{\tau, u, v}d(u, v) + 
 2 \sum_\tau\sum_v\sum_r x_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)$$, where $\Pr(z \sim P_\tau=r)$ denotes the probability that $r$ is requested at time $\tau$.
 \begin{equation}
 \begin{aligned}\nonumber
 & \text{min.} \hspace{1cm}
 && \sum_\tau\sum_{u, v}f_{\tau, u, v}d(u, v) + 
 2 \sum_\tau\sum_v\sum_r x_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)\\
 &\forall \tau, v	&& b_{\tau+1, v}=b_{\tau, v} + \sum_u f_{\tau, u, v} - \sum_u 
 f_{\tau, v, u}.\\
 &\forall \tau, u, v	&& \sum_v x_{\tau, v, r} \geq 1.\\
 &\forall \tau, v, r	&& x_{\tau, v, r} \leq b_{\tau, v}.\\
 &\forall \tau	&& \sum_v b_{\tau, v} \leq k.\\
 &\forall \tau, v, r	&& x_{\tau, v, r} \in \{0,1\}.\\
 &\forall \tau, u, v	&& f_{\tau, u, v} \in N.\\ 
 &\forall \tau, v	&& b_{\tau, v} \in N.\\ 
 \end{aligned}
 \end{equation}
 
%  to find a $t+1$ configurations $B_0$ to $B_t$ for a given sequence of $t$ distributions. 
Now we consider the following relaxation of the above integer program. Next, in Section \ref{fred} we show how a fractional solution can be rounded to an integral  solution.%$\tau+1$ we move the the 

\begin{equation}
\begin{aligned}\nonumber
& \text{min.} \hspace{1cm}
&& \sum_\tau\sum_{u, v}f_{\tau, u, v}d(u, v) + 
2 \sum_\tau\sum_v\sum_r x_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)\\
&\forall \tau, v	&& b_{\tau+1, v}=b_{\tau, v} + \sum_u f_{\tau, u, v} - \sum_u 
f_{\tau, v, u}.\\
&\forall \tau, u, v	&& \sum_v x_{\tau, v, r} \geq 1.\\
&\forall \tau, v, r	&& x_{\tau, v, r} \leq b_{\tau, v}.\\
 &\forall \tau	&& \sum_v b_{\tau, v} \leq k.
\end{aligned}
\end{equation}

%\subsection{Rounding}
%%In this section we provide a polynomial-time 3-approximation online algorithm for the stochastic k-server problem in the line metric. First we show that given a fractional algorithm with cost $M$, we can obtain a randomized integral algorithm with the expected cost of $M$. Then in subsection \ref{xxx}, we provide an optimal polynomial-time fractional request oblivious online algorithm. Then we can obtain an integral algorithm and use Theorem \ref{xxx} to achieve a 3-approximation online algorithm for the problem in the line metric.
%
%In this section we provide a rounding for the former relaxed linear program. Let $B$ denote a fractional configuration. Recall that on the line metric, for every $v \in V$, $B(v)$ denotes the amount of server mass on node $v$ of the line. For every fractional configuration $B$, we define a mass function $f_A: (0,k] \to V$ as follows.
%$f_B(x)=v_j$ if and only if $j$ is the minimum integer such that $\sum_{i=1}^{j-1} < x$ and $\sum_{i=1}^{j} \geq x$.
%%\snote{I should fix the definition.}
%Intuitively, if one gathers the server mass by sweeping the line from left to right, $f_B(x)$ is the position that we have gathered $x$ amount of server mass.
%%First we define function $\place_\tau(x):R \rightarrow V$ which denotes the place of server $x$ in configuration $A_{\tau}$. In particular, for a real number $x \in [0, k]$ and time step $\tau$, $\place_{\tau}(x)=u_j$ if and only if $\sum_{i=0}^{j-1}{X_{u_i}} < x$ and $\sum_{i=0}^{j}{X_{u_i}} \geq x$.
%%Now using function $\place$ we design our algorithm:
%
%\iffalse
%
%Now given a fractional algorithm $\afrac$ we provide the following integral algorithm.
%
%\begin{enumerate}
%	\item Pick a random real number $q \in (0, 1]$.
%	\item At each time step on realization of request $r$:
%	\begin{enumerate}
%		\item Let $B$ be the output configuration of $\afrac$ for $r$.
%		\item Place the $i$-th server on $f_{B}(i-1+q)$.
%	\end{enumerate}
%\end{enumerate}
%
%\fi
%
%Now we can define the rounding algorithm. First we pick a random real number $q \in (0, 1]$. For each time step $\tau$, let $B_\tau$ denote the fractional configuration obtained by the LP. Let $S_\tau=\langle s_1^\tau, \ldots, s_k^\tau \rangle$ be a sequence of $k$ nodes such that, $s_i^\tau=f_{B_\tau}(i-1+q)$.
%%Roughly speaking, we assume there are infinitely many servers each having infinitely small mass, such that their total mass is $k$, and choose $k$ of them in a randomized manner. Then the algorithm is to follow exactly this set of $k$ small servers. 
%%\snote{name of variables}.
%Now set each variable $b'_{\tau, v}$ to be an integer $i$ if and only if there are exactly $i$ number of $v$'s in $S_\tau$. For each possible request $r$ at time $\tau$ choose a node $v$ such that $v \in S_\tau$ and $x'_{\tau, r, v}>0$, then set $x_{\tau, v, r}=1$. %\snote{flow variables should be fixed}. 
%Now since all $b'_{\tau, u, v}$s are integers, there exists an integral assignment to movement variables $f_{\tau, u, v}$ such that the total movement is minimized. 
%% % % % % % % % % % % % % %
%
%% % % % % % % % % % % % % %
%
%In the following we prove the rounding provides a feasible solution (Lemma \ref{xxx}), and the expected cost of the solution equals the cost of the fractional solution (Lemma \ref{yyy}).
%
%%First we need the following observation.
%%\begin{observation}
%%	If for a configuration $A$ and two real numbers $x$ and $y$ $(y \geq x)$, $f_A(x)=f_A(y)=v$, then for every real number $z \in [x, y]$, $f_A(z)=v$.
%%\end{observation}
%\iffalse
%Observation \ref{xxX} follows directly from Observation \ref{xxx}.
%\begin{observation}
%Let $B$ be a fractional configuration $B$, and $B'$ be the corresponding rounded configuration. Then if there is a mass of server of size more than 1 on a node $v$ in $B$, then there is at least one server on $v$ in $B'$. In particular if $b_{\tau, v}\geq 1$, then $b'_{\tau, v} \geq 1$.
%\end{observation}
%\begin{proof}
%	 Let $v$ be a node such that $b_{\tau, v} \geq 1$. Let $x$ be the minimum real number such that $f_{B}(x)=v$. Similarly let $y$ be the maximum real number such that $f_B(y)=v$. Since there is a mass of size at least 1 on $v$, $y-x \geq 1$. Thus by Observation \ref{ooo} for any $z \in [x, y]$, $f_{B}(z)=v$. Note that $x, y \in (0, k]$ and thus for each real number $q \in (0, 1]$ there is an integer $i$ such that $0 \leq i \leq k-1$ and $x \leq i+q \leq y$. Thus by Observation \ref{ooo} $f_{B}(i+x)=v$. Therefore for any random value $q \in (0, 1]$ we place at , $\aint$ places the $l$-th server on $r_i$
%\end{proof}
%\fi
%\begin{lemma}
%%	Given an algorithm $\afrac$ which provides a fractional feasible solution for any sequence of requests $\rho=\langle r_0, \ldots, r_t\rangle$, $\aint$ provides an integral feasible solution for $\rho$. Algorithm $\aint $ always provides a feasible integral solution.
%The rounding provides a feasible solution for $k$-server on the line metric.
%\end{lemma}
%\begin{proof}
%	 %Let $opt$ be an optimal fractional solution for LP \ref{xxx}, and $sol'$ be the corresponding rounded integer solution. It is sufficient to prove $sol'$ is also a feasible solution for the LP. 
%	 Given an optimal solution for the relaxed LP, it is sufficient to prove that the corresponding integer solution obtained by the rounding is a feasible solution for the LP.
%	 
%	 
%	 We set each variable $b'_{\tau, v}$ to be an integer $i$ if and only if there are exactly $i$ number of $v$'s in $S_\tau$. Thus for each time step $\tau$, $\sum_{v \in V} b'_{\tau, v}=k$ and the forth set of constraints holds.
%	 	Now for a time step $\tau$ and possible request $r$, let $u$ be the leftmost node such that $x_{\tau, r, u} > 0$. Similarly let $v$ be the rightmost node such that $x_{\tau, r, v} > 0$. Since we consider an optimal solution, for every node $w \in V\setminus\{u, v\}$ between $u$ and $v$, $x_{\tau, r, w} = b_{\tau, w}$ %\snote{I should say there is no edge of size $0$}. 
%	 	Thus there are two real numbers $y_l, y_h \in (0, k]$ such that $y_h-y_l \geq 1$ and for every $y_l \leq y \leq y_h$, $x_{\tau, r, f(y)} > 0$. Therefore for any $q \in (0, 1]$ there is a node $v$ and an integer $i$ such that $y_l \leq i+q \leq y_h$ and $v =f_B(i+q)$. Thus $v \in S_\tau$, which implies 
%	 	 $b'_{\tau, v} \geq 1$ and $x_{\tau, v, r} = 1$. This means the second and third sets of constraints hold for the integer solution we provided. In particular, 
%	 	 	 for every $r, v \in V$ and $1 \leq \tau \leq t$, $\sum_{v\in V}x'_{\tau, v, r} \geq 1$ and $x'_{\tau, v, r} \leq b'_{\tau, v}$. 
%	 	 	 
%	 	  %a consecutive mass of size at least one going that serves $r$. Thus there is There is a mass of size at least 1 on $v$, $y-x \geq 1$. Thus by Observation \ref{ooo} for any $z \in [x, y]$, $f_{B}(z)=v$. Note that $x, y \in (0, k]$ and thus for each real number $q \in (0, 1]$ there is an integer $i$ such that $0 \leq i \leq k-1$ and $x \leq i+q \leq y$. Thus by Observation \ref{ooo} $f_{B}(i+x)=v$. Therefore for any random value $q \in (0, 1]$ we place at , $\aint$ places the $l$-th server on $r_i$
%	 	 
%	 %Recall that a fractional feasible solution for $\rho$ is a sequence of configurations $\langle A_{f0}, \ldots, A_{ft}\rangle$, such that in $A_j$ there is a mass of server assigned to point $r_j$ of size at least 1 i.e., $A_j(r_j) \geq 1$. For an integral feasibility, we need to prove $\aint$ provides a sequence of configurations $\langle A_{i0}, \ldots, A_{it}\rangle$ such that there exists a server on point $r_j$ in configuration $A_{ij}$.
%	 %Now for a request $r_j$ consider the fractional configuration $A_{fj}$. Let $x$ be the minimum real number such that $f_{A_{fj}}(x)=r_j$. Similarly let $y$ be the maximum real number such that $f_{A_{fj}}(y)=r_i$. . Since there is a mass of size at least 1 on $r_j$, $y-x \geq 1$. Thus by Observation \ref{ooo} for any $z \in [x, y]$, $f_{A_{fj}}(z)=r_i$. Note that $x, y \in (0, k]$ and thus for each real number $q \in (0, 1]$ there is an integer $l$ such that $0 \leq l \leq k-1$ and $x \leq l+q \leq y$. Thus by Observation \ref{ooo} $f_{A_{fj}}(l+x)=r_i$. Therefore for any random value $q \in (0, 1]$, $\aint$ places the $l$-th server on $r_i$. Thus it serves $r_i$ and provides a feasible integral solution.
%\end{proof}
%
%For Lemma $\ref{xxx}$, we need the following proposition.
%\begin{proposition}
%For two fractional configurations $B_1$ and $B_2$, $d(B_1, B_2)=\int_{0^+}^k d(f_{B_1}(x), f_{B_2}(x))dx$.
%\end{proposition}
%%\snote{I'm not sure if it needs a proof}
%\begin{lemma}
%	%Given an algorithm $\afrac$ for a sequence of requests $\rho=\langle r_0, \ldots, r_t\rangle$, with cost $m$. $\aint$, algorithm $\aint $ has an expected cost $m$.
%	The integrality gap of LP \ref{xxx} is 1.
%\end{lemma}
%\begin{proof}
%	By Proposition \ref{xxx}, 
%	\begin{equation}
%	\begin{aligned}
%		d(B_{i}, B_{i+1})&=\int_{x=0^+}^k
%		 d(f_{B_{i}}(x), f_{B_{i+1}}(x))dx.\nonumber\\
%		&=\int_{x=0^+}^1 \sum_{i=0}^{k-1} d(f_{B_{i}}(x), f_{B_{i+1}}(x))dx.
%	\end{aligned}
%	\end{equation}
%	Now let $B'_{i-1}$ and  $B'_i$ denote the rounded integral configurations for $B_{i-1}$ and $B_i$, and $q\in(0, 1]$ be a random real number. Thus
%	\begin{equation}
%		d(B'_{i}, B'_{i+1})= \sum_{i=0}^{k-1} d(f_{B'_{i}}(i+q), f_{B'_{i+1}}(i+q)).
%	\end{equation}
%	Thus the expected value for $d(B'_{i-1}, B'_i)$ is
%	\begin{equation}
%	E[d(B'_{i}, B'_{i+1})] = \int_{q=0^+}^k\sum_{i=0}^{k-1} d(f_{B'_{i}}(i+q), f_{B'_{i+1}}(i+q))dq = d(B_{i}, B_{i+1}).
%	\end{equation}
%	Similarly, for each fractional configuration $B$ and request $r$, there is a continuous mass of size 1, serving $r$, thus the cost for serving $r$ in $B$ is
%	\begin{equation}
%	\int_{x=z^+}^{z+1}d(f_B(x), r)dx.
%	\end{equation}
%		The integral solution considers a random $q \in (0, 1]$ such that $i+q \in (z, z+1]$, hence the expected cost of integral solution is $\int_{x=z^+}^{z+1}d(f_{B}(x), r)dx.$		
%	Thus by Equations \eqref{xxx} and \eqref{yyy}, 
%	\begin{equation}
%	\begin{aligned}
%	&\sum_\tau\sum_{u, v}f_{\tau, u, v}d(u, v) + 
%	2 \sum_\tau\sum_v\sum_r x_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)=\\
%	&\sum_\tau d(B_\tau, B_{\tau+1}) + 
%	2 \sum_\tau\sum_r \Pr(z \sim P_\tau=r)\int_{x=z_{\tau, r}^+}^{z_{\tau+1, r}}d(f_{B_\tau}(x), r)dx=\\
%	&E[\sum_\tau d(B'_\tau, B'_{\tau+1}) + 
%	2 \sum_\tau\sum_r \Pr(z \sim P_\tau=r)\int_{x=z_{\tau, r}^+}^{z_{\tau+1, r}}d(f_{B_\tau}(x), r)dx]=\\
%	&E[\sum_\tau\sum_{u, v}f'_{\tau, u, v}d(u, v) + 
%	2 \sum_\tau\sum_v\sum_r x'_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)].
%	\end{aligned}
%	\end{equation}
%
% Thus in expectation the integral solution has equal cost to the fractional solution. Since we considered an optimal fractional solution, for any $q$ this equality holds, hence
% \begin{equation}
% \begin{aligned}
%&\sum_\tau\sum_{u, v}f_{\tau, u, v}d(u, v) + 
% 2 \sum_\tau\sum_v\sum_r x_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r)=\\
% &\sum_\tau\sum_{u, v}f'_{\tau, u, v}d(u, v) + 
% 2 \sum_\tau\sum_v\sum_r x'_{\tau, v, r}\Pr(z \sim P_\tau=r)d(v, r).
% \end{aligned}
% \end{equation}
%		%E[d(B'_{i-1}, B'_i)] = \int_{q=0^+}\sum_{i=1}^k d(f_{B'_{i-1}}(i+q), f_{B'_{i}}(i+q))dq = d(B_{i-1}, B_i).
%\end{proof}
%
%\begin{theorem}
%	There exists a polynomial time algorithm which finds the optimal non-adaptive  online algorithm for the stochastic $k$-server problem on the line metric.
%\end{theorem}
% 
%The following Theorem follows directly from Theorems \ref{xxx} and \ref{yyy}.
%\begin{theorem}
%	There exists a polynomial time 3-approximation algorithm for the stochastic $k$-server problem on the line metric
%\end{theorem}
%\newpage

==> general_graph_to_hst.tex <==
\subsection{Embedding General Metrics Into HSTs}
Embedding general metrics into trees and in particular HSTs has been the subject of many studies. The seminal work of \ref{fakcharoenphol2003tight}

==> log4.tex <==
In this section we present a poly-logarithmic competitive ratio algorithm for \odbsf{}. To do so, we first find a fractional solution for Linear Program \eqref{LP:sf} with an $O(log^2(n))$ violation on the degree constraints and the weight constraint. In this LP we assume that we are given the weight of the optimal Steiner forest $w(opt)$. In the actual execution of the algorithm we do not know the value of $w(opt)$. Therefore, we begin with a small enough initial guess for $w(opt)$. Whenever the algorithm violates one of the packing constraints with more that the allowed violation, we rerun the algorithm from the beginning with a new guess for $w(opt)$. In theorem XXX, we show how this doubling technique results in loosing a factor of $O(log(n))$ only for the degree bound constraints. Finally Theorem \ref{thm:rounding} shows our rounding algorithm preserves the same violation factors as of the fractional LP.

\subsection{Fractional Solution}

Let $\sigma$ denote the sequence of demands. For every demand $(s_i, t_i)\in \sigma$ we define a collection $\mathcal{S}_i$ of the subsets of $V$. This collection contains a set of vertices $S\subseteq V$ if and only if $S$ separates $s_i$ from $t_i$ and $S$ does not separate any other $s_j$ and $t_j$ for a previously satisfied demand $j<i$.

As indicated for \ref{IP:sf}, when a new demand $(s_i, t_i)$ arrives, we have to ensure that for every $S\in\mathcal{S}$ that separates $s_i$ from $t_i$, there is an outgoing edge from $S$ in $H_i$. Note that if such $S$ is also a separating set for some other demand $(s_j, t_j)$, $j<i$, then there already exists an outgoing edge from $S$ in $H_j\subseteq H_i$. Therefore the corresponding covering constraint is already satisfied when demand $i$ arrives. We use this fact and write new covering constraints in \ref{LP:sf} only for every $S\in\mathcal{S}_i$.

By the definition, $w(opt)$ is the minimum weight of a solution satisfying all degree bound constraints. Therefore, the optimal offline solution to \ref{LP:sf} is $1$.

\begin{align*}
\text{minimize}           &\quad \quad \alpha \tag{{$\mathbb{LP}1$}}\label{LP:sf}\\
\forall v \in V &\quad\quad  \frac{1}{b_v}\sum_{i\leq |\sigma|}^{}\sum_{e \in \delta(v)}{x_e^i} \leq \alpha\\
&\quad\quad \frac{1}{w(opt)}\sum_{i\leq |\sigma|}^{}\sum_{e \in E}w(e)x_e^i \leq \alpha \\
\forall i \leq |\sigma|, S \in \mathcal{S}_i &\quad\quad \sum_{e \in \delta(S)} {x_e^i} \geq 1 \\
&\quad\quad \x, \alpha \geq 0
\end{align*}

\begin{corollary} \label{cor:opt=1}
	Let $\alpha_{opt}$ be the optimal solution to \eqref{LP:sf}. $\alpha_{opt}=1$.
\end{corollary}

All packing constraints can be written before the arrival of the first demand. When a new demand $i$ comes, we have to increase $\x$ such that the set of constraint of type $\sum_{e \in \delta(S)} {x_e^i} \geq 1$ are covered for every $S\in \mathcal{S}_i$. To simplify the online scenario, assume that these covering constraints are coming one by one, and we have to satisfy every constraint before the arrival of the next constraint.

Let $m=n+1$ be the number of packing constraints and $d=|E|.|\sigma|$ be the number of variables in $\x$. Define $\mu=1+\frac{1}{3\ln(em)}$ and $\rho = e^2 \ln(\mu d max\{w(e)\})$. Note that assuming all edge weights are natural numbers and the maximum weight is a polynomial of $n$, then $\rho \in O(log(n))$. We divide every coefficient in packing constraints by $2\rho$. Note that based on Corollary \ref{cor:opt=1} the optimal of the new LP \eqref{LP_scaled_primal} is $\frac{1}{2\rho}$. Now we use primal-dual technique to find a solution of at most $3\ln(em)$ for the scaled LP. Lemma \ref{lm:main} shows our result is $O(log^2(n))$ competitive.

\noindent
%\begin{minipage}{.44\textwidth} %
\begin{align}
\text{minimize}  &\quad \alpha \tag{{$\mathbb{P}$}}\label{LP_scaled_primal}\\ \label{deg_bound_constraint}
\forall v \in V &\quad  \frac{1}{2\rho}\frac{1}{b_v}\sum_{i=1}^{|\sigma|}\sum_{e \in \delta(v)}{x_e^i} \leq \alpha\\ \label{weight_bound_constraint}
&\quad \frac{1}{2\rho}\frac{1}{w(opt)}\sum_{i=1}^{|\sigma|}\sum_{e \in E}w(e)x_e^i \leq \alpha \\
\forall i \leq |\sigma|, S \in \mathcal{S}_i &\quad \sum_{e \in \delta(S)} {x_e^i} \geq 1 \\ \nonumber
&\quad \x, \alpha \geq 0 \nonumber
\end{align}
%\end{minipage} %
%\hspace{0.02\textwidth}
%\begin{minipage}{.53\textwidth} %
\begin{align}
\text{maximize} &\quad  \sum_{i=1}^{|\sigma|}\sum_{S\in \mathcal{S}_i}{y_{S}^{i}} \tag{{$\mathbb{D}$}}\label{LP_scaled_dual}\\ \label{ineq:dual1}
\forall e=(u,v), i\leq |\sigma| &\quad \sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \frac{z_u}{2\rho b_u}+\frac{z_v}{2\rho b_v}+\frac{w(e) z_w}{2\rho w(opt)}\\ \label{ineq:dual2}
&\quad  z_w + \sum_{v=1}^{n}{z_v} \leq 1 \\
&\quad  \z, \y \in \mathbb{\sigma}_{\geq 0}
\end{align}
%\end{minipage}

In the dual LP \ref{LP_scaled_dual} every variable $z_1,\ldots,z_n$ and $z_w$ corresponds to one of the constraints in \ref{deg_bound_constraint} and \ref{weight_bound_constraint} respectively. In our proofs we use $z_w$ and $z_{n+1}$ interchangeably. A dual variable $y_{S}^{i}$ is corresponding to a covering constraint defined by $S\in\mathcal{S}_i$ of demand $i$.

For a given vector of variables $\x$ and $1\leq k \leq m$, let $\alpha_k(\x)$ be value of the left hand side of packing constraint $k$, where $\alpha_{n+1}(\x)$ corresponds to \eqref{weight_bound_constraint}. Let $\alpha(\x)=\max_{1\leq k\leq m}\{\alpha_k(\x)\}$. Our goal is to find a feasible $\x$ that minimizes $\alpha(\x)$.

The potential function $\Phi(\x)$ is defined as follows
$$\Phi(\x) := \ln\big( \sum_{k=1}^{m}\exp(\alpha_k(\x)) \big) \enspace .$$
Since $\alpha(\x)\leq \Phi(\x) \leq \alpha(\x)+\ln(m)$, we use this potential function as an estimate of $\alpha(\x)$.

% make sure that the modification you made does not hurt the whole proof

The algorithm initializes the variables with a vector $\x^0$ with $1/(d \max_{e\in E}\{w(e)\})$ for each variable $x_{e}^{i}$, $e\in E$ and $1\leq i\leq |\sigma|$.

\begin{lemma}
	$\Phi(\x^0) \leq 1/(2\rho) + \ln(m)$.
\end{lemma}
\begin{proof}
	For every packing constraint $1 \leq v \leq n$:
	$$\alpha_v(\x^0) \leq d \frac{1}{d\max_{e\in E}\{w(e)\}} \frac{1}{2\rho b_v}\leq \frac{1}{2\rho} \enspace .$$
	For constraint $n+1$:
	$$\alpha_{n+1}(\x^0) \leq d \frac{1}{d\max_{e\in E}\{w(e)\}}\frac{\max_{e\in E}\{w(e)\}}{2\rho w(opt)} \leq \frac{1}{2\rho} \enspace .$$
	Hence,
	$$\Phi(\x^0) = \ln\big( \sum_{k=1}^{n+1}\exp(\alpha_k(\x^0)) \big) \leq \ln\big(\sum_{k=1}^{m}\exp(1/(2\rho))\big) \leq \frac{1}{2\rho} + \ln(m) \enspace .$$
\end{proof}

To satisfy a new covering constraint we do multiplicative updates on every variable. For every $e=(u,v)\in E$ and $1\leq i\leq |\sigma|$, define
\begin{align*}
rate_{e,i}(\x) = \frac{\partial \Phi(\x)}{\partial x_{e}^{i}}&=\frac{e^{\alpha_u(\x)}/(2\rho b_u)+e^{\alpha_v(\x)}/(2\rho b_v)+e^{\alpha_w(\x)}w(e)/(2\rho w(opt))}{ \sum_{k=1}^{m}e^{\alpha_k(\x)}} \\
&= \frac{e^{\alpha_u(\x)}/b_u+e^{\alpha_v(\x)}/b_v+e^{\alpha_w(\x)}w(e)/w(opt)}{ 2\rho\sum_{k=1}^{m}e^{\alpha_k(\x)}} \enspace .
\end{align*}

For a covering constraint corresponding to $S\in \mathcal{S}_i$ of demand $i$, define
$$\epsilon_{S}^{i}(\x) = (\mu-1)\min_{e\in\delta(S)}\{rate_{e,i}(\x)\}$$
so that for all $e \in \delta(S)$, $\epsilon_{S}^{i}(\x) / rate_{e,i}(\x) \leq \mu-1$. For this covering constraint there is a variable $y_{S}^{i}$ in the dual LP \eqref{LP_scaled_dual}. Repeat the following steps until the constraint is satisfied ($\sum_{e \in \delta(S)} {x_e^i} \geq 1$).
\begin{itemize}
	\item Let $\x^l$ be the current value of variables in \eqref{LP_scaled_primal}.
	\item For each $e\in \delta(S)$, multiply $x_{e}^{i}$ by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$.
	\item Add $e\epsilon_{S}^{i}(\x^l)$ to dual variable $y_{S}^{i}$.
\end{itemize}

A single iteration of the above loop is called a \textit{phase} indexed by $l$. Let $L_{S}^{i}$ be the set of all phases executed for constraint $S\in\mathcal{S}_i$ of demand $i$, and $L=\cup L_{S}^{i}$. Note that in every phase variables are multiplied by a factor of at most $\mu$.

\begin{lemma}
	\label{rate_ratio}
	For a given $\x$ and $\x'$ with $\alpha(\x)\leq 3\ln(m)$, if $x_{e}^{i} \leq x_{e}^{\prime i} \leq \mu x_{e}^{i}$ for every $1\leq i \leq |\sigma|$ and $e\in E$, then
	$$rate_{e, i}(\x') \leq e \, \text{rate}_{e, i}(\x) \enspace .$$
\end{lemma}

\begin{proof}
	Since $\alpha_k(\x)\leq \alpha(\x) \leq 3\ln(em)$,
	\begin{align*}
	\mu \alpha_k(\x)
	\leq \bigg(1+\frac{1}{3\ln(em)}\bigg)\alpha_k(\x)
	\leq \alpha_k(\x)+\frac{\alpha_k(\x)}{3\ln(em)}
	\leq \alpha_k(\x)+\frac{\alpha(\x)}{3\ln(em)}
	\leq \alpha_k(\x)+1 \enspace .
	\end{align*}
	By the linearity of constraints,
	\begin{align}
	\label{ineq1}
	\forall k: \quad\quad \alpha_k(\x) \leq \alpha_k(\x') \leq 	\mu \alpha_k(\x)  \leq \alpha_k(\x)+1 \enspace .
	\end{align}
	Using \ref{ineq1} in the definition of $rate_{e,i}(\x')$,
	\begin{align*}
	rate_{e,i}(\x')&= \frac{e^{\alpha_u(\x')}/b_u+e^{\alpha_v(\x')}/b_v+e^{\alpha_w(\x')}w(e)/w(opt)}{ 2\rho\sum_{k=1}^{m}e^{\alpha_k(\x')}}
	\\
	&\leq
	\frac{e^{\alpha_u(\x)+1}/b_u+e^{\alpha_v(\x)+1}/b_v+e^{\alpha_w(\x+1)}w(e)/w(opt)}{ 2\rho\sum_{k=1}^{m}e^{\alpha_k(\x+1)}} \\
	&= e \bigg ( \frac{e^{\alpha_u(\x)}/b_u+e^{\alpha_v(\x)}/b_v+e^{\alpha_w(\x)}w(e)/w(opt)}{ 2\rho\sum_{k=1}^{m}e^{\alpha_k(\x)}}
	\bigg ) \\
	&= e \, rate_{e, i}(\x) \enspace .
	\end{align*}
\end{proof}

\begin{lemma}
	The increase in $\sum_{i=1}^{|\sigma|}\sum_{S\in \mathcal{S}_i}{y_{S}^{i}}$ is an upper bound for the total increase in $\Phi(\x)$.
\end{lemma}

\begin{proof}
	To prove the lemma we show that in every phase $l$ the amount of increase in the potential function, $\Phi(\x^{l+1})-\Phi(\x^l)$, is at most the amount of increase in the corresponding dual variable $y_{S}^{i}$. Suppose that at this phase $l$, the algorithm is trying to satisfy a covering constraint $S\in\mathcal{S}_i$of demand $1\leq i\leq |\sigma|$. We show that the amount of increase in the potential function is at most $e\epsilon_{S}^{i}(\x^l)$.
	
	Let $\x(t):=\x^l + (\x^{l+1}-\x^l)t$ for $0\leq t\leq 1$. Base on this function, we can define $\phi(t):=\Phi(\x(t))$ and $rate_{e,i}(t):=rate_{e,i}(\x(t))$. The derivative of $\phi(t)$ is 
	\begin{align}
	\frac{\partial \phi(t)}{\partial t} = \sum_{e\in \delta(S)} \frac{\partial \phi(t)}{\partial x_{e}^{i}(t)}\frac{\partial x_{e}^{i}(t)}{\partial t} = \sum_{e\in\delta(S)} rate_{e,i}(t)\frac{\partial x_{e}^{i}(t)}{\partial t} \enspace .
	\end{align}
	From lemma \ref{rate_ratio} we have $rate_{e,i}(t)\leq e\, rate_{e,i}(0)=e \, rate_{e,i}(\x^l)$. Therefore,
	\begin{align}
	\nonumber
	\Phi(\x^{l+1})-\Phi(\x^l) &= \int_{0}^{1} \frac{\partial \phi(t)}{\partial t} dt \\ \nonumber
	&= \int_{0}^{1} \sum_{e\in \delta(S)} rate_{e,i}(t)\frac{\partial x_{e}^{i}(t)}{\partial t} dt\\ \nonumber
	&\leq e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\int_{0}^{1} \frac{\partial x_{e}^{i}(t)}{\partial t} dt\\ \nonumber
	&=  e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i}(1)-x_{e}^{i}(0)\big) \\ \label{diff_x}
	&=  e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i,l+1}-x_{e}^{i,l}\big) \enspace .
	\end{align}
	Recall that in phase $l$ we multiply $x_{e}^{i}$ by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$  for every $e\in\delta(S)$. Hence, the difference between $x_{e}^{i,l+1}$ and $x_{e}^{i,l}$ in \eqref{diff_x} is exactly $x_{e}^{i,l}\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l)$.
	\begin{align}
	\nonumber
	\Phi(\x^{l+1})-\Phi(\x^l) &\leq e \sum_{e\in\delta(S)}rate_{e,i}(\x^l)\big( x_{e}^{i,l+1}-x_{e}^{i,l}\big) \\ \nonumber
	&= e\,\epsilon_{S}^{i}(\x^l)\sum_{e\in\delta(S)}x_{e}^{i,l}\\
	&\leq e\,\epsilon_{S}^{i}(\x^l) \enspace .
	\end{align}
	The last inequality holds because the covering constraint is not satisfied before the execution of phase $l$.
\end{proof}

\begin{lemma}
	For every $e\in E$ and $1\leq i\leq |\sigma|$,
	$$\sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \rho \max_{l\in L}\{rate_{e,i}(x^l)\} \enspace .$$
\end{lemma}

\begin{proof}
	In every phase $l$, $x_{e}^{i}$ is multiplied by $1+\epsilon_{S}^{i}(\x^l)/rate_{e,i}(\x^l) \geq \exp\bigg(\frac{\epsilon_{S}^{i}(\x^l)}{e\,rate_{e,i}(\x^l)}\bigg)$, where the inequality comes from $1+a\geq\exp(a/e)$ for $0\leq a\leq 1$. Moreover, the initial value of $x_{e}^{i}$ is $1/(d\max_{e\in E}\{w(e)\})$ and will never exceed $\mu$, because otherwise $x_{e}^{i}$ satisfies the phase termination condition.
	$$
	\frac{1}{d\max_{e\in E}\{w(e)\}}\prod_{S\in\mathcal{S}_i:e\in\delta(S)}\prod_{l\in L_{S}^{i}}\exp\bigg(\frac{\epsilon_{S}^{i}(\x^l)}{e\,rate_{e,i}(\x^l)}\bigg) \leq x_{e}^{i} \leq \mu \enspace .
	$$
	By multiplying both sides by $d\max_{e\in E}\{w(e)\}$ and taking natural log, 
	$$
	\label{ineq:vasati}
	\sum_{S\in\mathcal{S}_i:e\in\delta(S)}\sum_{l\in L_{S}^{i}}\frac{{\epsilon_{S}^{i}(\x^l)}}{e\,rate_{e,i}(\x^l)}
	\leq \ln\big(\mu d \max_{e\in E}\{w(e)\}\big ) \enspace .
	$$
	By multiplying both sides by $e\,\max_{l\in L}\{rate_{e,i}(\x^l)\}$ we get
	\begin{align}
	\label{ineq:sakhte}
	\sum_{S\in\mathcal{S}_i:e\in\delta(S)}\sum_{l\in L_{S}^{i}}{\epsilon_{S}^{i}(\x^l)} \leq e\,\ln\big(\mu d \max_{e\in E}\{w(e)\}\big) \max_{l\in L}\{rate_{e,i}(\x^l)\} \enspace .
	\end{align}	
	From the updates of the algorithm, a dual variable $y_{S}^{i}$ is exactly $e\sum_{l\in L_{S}^{i}}\epsilon_{S}^{i}(\x^l)$. On the other hand $\rho\geq	e^2\,\ln(\mu d \max_{l\in L}\{rate_{e,i}(\x^l)\})$, therefore by multiplying both sides of Inequality \ref{ineq:sakhte} by $e$ we have
	\begin{align}
	\label{ineq:sakhe_final}
	\sum_{S\in\mathcal{S}_i:e\in\delta(S)}y_{S}^{i} \leq \rho \max_{l\in L}\{rate_{e,i}(\x^l)\} \enspace .
	\end{align}
\end{proof}


Now we set dual variables $z_k$ so that for every $e=(u,v)\in E$ and $1\leq i \leq |\sigma|$ the right hand side of \eqref{ineq:dual1}  is at least $\max_{l\in L}\{rate_{e,i}(\x^l)\}$. This makes every constraint in \eqref{ineq:dual1} being violated by a factor of at most $\rho$.

By the definition,

\begin{align*}
\max_{l\in L}\{rate_{e,i}(\x^l)\} &= \max_{l\in L}\bigg\{\frac{e^{\alpha_u(\x^l)}/b_u+e^{\alpha_v(\x^l)}/b_v+w(e)e^{\alpha_w(\x^l)}/w(opt)}{\rho \sum_{k=1}^{m}e^{\alpha_k(\x^l)}}\bigg\} \\
&\leq \frac{1}{\rho b_u}\max_{l\in L}\bigg\{\frac{e^{\alpha_u(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} +
\frac{1}{\rho b_v}\max_{l\in L}\bigg\{\frac{e^{\alpha_v(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} +
\frac{w(e)}{\rho w(opt)}\max_{l\in L}\bigg\{\frac{e^{\alpha_w(\x^l)}}{\sum_{k=1}^{m}e^{\alpha_k(x^l)}}\bigg\} \enspace .
\end{align*}

Therefore, setting $z_k=\max_{l\in L}\bigg\{\frac{\exp(\alpha_k(\x^l))}{\sum_{k'=1}^{m}\exp(\alpha_{k'}(\x^l))}\bigg\}$ for every $k$ attains our goal.

\begin{corollary} \label{cor:dual_violation}
	For every $e=(u,v)\in E$ and $1\leq i\leq |\sigma|$,
	$$ \sum_{S\in \mathcal{S}_i:e\in \delta(S)}{y_{S}^{i}} \leq \rho\bigg(\frac{z_u}{2\rho b_u}+\frac{z_v}{2\rho b_v}+\frac{w(e) z_w}{2\rho w(opt)}\bigg) \enspace .$$
\end{corollary}

In the following lemma, we find an upper bound for the left hand side of \eqref{ineq:dual2}. This upper bound is later used in Lemma \ref{lm:main} to construct a solution for the dual LP.

\begin{lemma} \label{lm:dual_ineq2}
	
	$\label{ineq:dual_ineq2}
	\sum_{k=1}^{m} z_k \leq \ln(em) + \max_{l\in L}\{\alpha(\x^l)\} \enspace .$
\end{lemma}

\begin{proof}
	For each packing constraint $k$, define
	$$\ind(k) := \argmax_{l\in L}\bigg\{\frac{e^{\alpha_k(\x^l)}}{\sum_{k'=1}^{m}e^{\alpha_{k'}(\x^l)}}\bigg\} \enspace .$$
	Thus $\ind(k)$ is the phase in which $z_k$ attains its value. Without loss of generality, we reorder the packing constraints in \ref{LP_scaled_primal} such that $\ind(l)<\ind(k)$ for every $l<k$. We use the following bound in order to prove the lemma.
	\begin{lemma} [Azar et al. \cite{XXX}] \label{lm:azar_khanum}
		For $m\in \mathbb{Z}_{+}$ and $a_1,\ldots,a_m \in \mathbb{\sigma}_{\geq 0}$ with $a_1>0$, $$\sum_{i=1}^{m}\frac{a_i}{\sum_{j\leq i}a_j} \leq 1 + \ln\bigg (\frac{\sum_{i=1}^{m}a_i}{a_1} \bigg) \enspace . $$
	\end{lemma}
	
	Let $a_k:=\exp(\alpha_k(\x^{\ind(k)}))$. Since the primal variables are non-decreasing in time, $\alpha_l(x^{\ind(k)})\geq \alpha_l(x^{\ind(l)})$. Therefore for every $k$,
	\begin{align}
	\label{ineq:zkak}
	z_k &= \frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{m}\exp(\alpha_{l}(\x^{\ind(k)}))}
	\leq \frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{k}\exp(\alpha_{l}(\x^{\ind(k)}))}
	\leq
	\frac{\exp(\alpha_k(\x^{\ind(k)}))}{\sum_{l=1}^{k}\exp(\alpha_{l}(\x^{\ind(l)}))}
	=\frac{a_k}{\sum_{l\leq k}a_l} \enspace .
	\end{align}
	From Inequality \eqref{ineq:zkak} and Lemma \ref{lm:azar_khanum} we have
	\begin{align} \label{ineq:p1}
	\sum_{k=1}^{m}z_k\leq \sum_{k=1}^{m}\frac{a_k}{\sum_{l\leq k}a_l} \leq 1 + \ln\bigg (\frac{\sum_{k=1}^{m}a_k}{a_1} \bigg) \enspace .
	\end{align}
	Considering the fact that $\alpha_1(\x^{\ind(1)})\geq 0$, and $a_1\geq 1$,
	\begin{align} \label{ineq:p2}
	1 + \ln\bigg (\frac{\sum_{k=1}^{m}a_k}{a_1} \bigg) \leq 1 + \ln\big (\sum_{k=1}^{m}a_k\big) \leq 1 + \ln(m) + \ln\big(\max_{k}(a_k)\big) \enspace .
	\end{align}
	By the definition of $a_k$,
	\begin{align} \label{ineq:p3}
	1 + \ln(m) + \ln\big(\max_{k}(a_k)\big) \leq \ln(em) + \ln\big(\max_{l}\big(\exp(\alpha(\x^l))\big)\big) \leq \ln(em) + \max_{l\in L}(\alpha(\x^l)) \enspace .
	\end{align}
	The proof follows from the Inequalities \eqref{ineq:p1}, \eqref{ineq:p2}, and \eqref{ineq:p3}.
\end{proof}

%Using Corollary \ref{cor:dual_violation} and Lemma \ref{lm:dual_ineq2} we make a feasible solution dual LP \ref{LP_scaled_dual}.

Using the previous lemmas we can now prove an upper bound on the competitive ratio of the algorithm.

\begin{lemma} \label{lm:main}
	The algorithm is $6\rho\ln(em)$-competitive.
\end{lemma}

\begin{proof}
	Define $\nu:=\ln(em)+\alpha(\x^l)$. The dual problem is a maximization problem, and Corollary \ref{cor:dual_violation} and Lemma \ref{lm:dual_ineq2} show that $\z/\nu$ and $\y/(\rho\nu)$ are feasible values for the dual variables. By weak duality, any feasible dual solution is a lower bound on the optimal primal solution $\hat{\alpha_{opt}}$. Based on Corollary \ref{cor:opt=1}, the optimal solution to \ref{LP_scaled_primal} is $\hat{\alpha_{opt}}=\frac{1}{2\rho}$. Hence $\sum_{i=1}^{|\sigma|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}/(\rho\nu)\leq \frac{1}{2\rho}$. The dual objective $\sum_{i=1}^{|\sigma|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}$ is an upper bound on the total increase in $\Phi(\x)$. At the beginning, $\Phi(\x^0)\leq \frac{1}{2\rho}+\ln(m)$. $\Phi(\x)$ is itself an upper bound for $\alpha(\x)$. Therefore,
	\begin{align} \label{ineq:upperbound}
	\alpha(\x)\leq \frac{1}{2\rho}+\ln(m)+\sum_{i=1}^{|\sigma|}\sum_{S\in\mathcal{S}_i}y_{S}^{i}\leq \frac{1}{2\rho}+\ln(m)+\frac{\nu}{2} \enspace .
	\end{align}
	
	Substituting $\nu=\ln(em)+\alpha(\x)$ yields $\alpha(\x)\leq 3\ln(em)$, and $\nu=\ln(em)+\alpha(\x)\leq 4\ln(em)$. Considering $\hat{\alpha_{opt}}=\frac{1}{2\rho}$ and plugging in the upper bound of $\nu$ in Inequality \eqref{ineq:upperbound} the competitive ratio of the algorithm is obtained.
	
	\begin{align*}
	\alpha(\x) &\leq \frac{1}{2\rho}+\ln(m)+\frac{\nu}{2} \\
	&\leq \hat{\alpha_{opt}} + 2\rho\ln(m) \hat{\alpha_{opt}} + 4\rho\ln(em)\hat{\alpha_{opt}} \\
	&\leq 6\rho\ln(em)\hat{\alpha_{opt}} \enspace .
	\end{align*}	
\end{proof}

\subsection{Rounding}

In the previous section we showed how to find a fractional solution $\x$ to \ref{LP:sf} that violates the degree bound and the weight constraints with a factor of $O(log^2(n))$. In this section we show how we use that solution to select a new set of edges that ensures the connection between the recently arrived demand $(s_i, t_i)$.

Let $H_i$ denote our solution after the satisfaction of demand $i$, and $H=\cup H_i$. From the fractional solution of \ref{LP_scaled_primal}, whenever a new demands $i$ arrives, we satisfy a set of covering constraints of type $\sum_{e\in\delta(S)}x_{e}^{i}\geq 1$ for every $S\in\mathcal{S}_i$. These constraints ensure the existence of a path from $s_i$ to $t_i$ using edges of $H_{i-1}$ and every $e$ with $x_{e}^{i}>0$. Let $P_{i, 1}$ denote the set of all edges $e$ in that path for which $x_{e}^{i}>0$, and $f(P_{i, 1})=\min_{e\in P_{i,1}}\{x_{e}^{i}\}$. Therefore, $P_{i,1}$ is in general a sequence of paths. Without loss of generality we assume $P_{i,1}$ has no cycle. We extract $P_{i,1}$ from $\x$ by decreasing $f(X_{P_{i,j}})$ from $x_{e}^{i}$ for every $e\in P_{i,1}$, and similarly find other paths $P_{i,2}$ to $P_{i, l_i}$ such that $\sum_{j=1}^{l_i}f(P_{i,j})=1$. In this way, for every edge $e\in E$
$$\sum_{P_{i,j}:e\in P_{i,j}}f(P_{i,j})\leq x_{e}^{i}\enspace .$$

We now select exactly one of $P_{i,1},\ldots,P_{i,l_i}$ such that the probability of each $P_{i,j}$ being selected is $f(P_{i,j})$. When a $P_{i,j}$ is selected we add all of its edges to $H_i$. This ensures the connection between $s_i$ and $t_i$. However, we need to show that with high probability the expectation of degrees and the expectation of weight are bounded.

\begin{theorem} \label{thm:rounding}
	Knowing $w(opt)$, our rounding algorithm is $O(log^2(n))$-competitive in expectation, while with high probability every degree bound is violated with at most $O(log^2(n))$.
\end{theorem}

\begin{proof}

	Let $X_{P_{i,j}}$ be a binary random variable with $1$ if $P_{i,j}$ is selected. For every $v\in V$, the expectation of the violation of $deg_H(v)$ is:

	\begin{align*}
		E_v = E\bigg[\frac{deg_H(v)}{b_v}\bigg] \leq 2 E\bigg[\frac{1}{b_v}\sum_{i=1}^{|\sigma|}\sum_{j:v\in P_{i, j}}X_{P_{i,j}}\bigg] = \frac{2}{b_v}\sum_{i=1}^{|\sigma|}\sum_{j:v\in P_{i, j}}f(P_{i,j}) \leq \frac{2}{b_v}\sum_{i=1}^{|\sigma|}\sum_{e\in\delta(v)}x_{e}^{i} \in O(log^2(n)) \enspace .
	\end{align*}

	Since $X_{P_{i,j}}$'s are not positively correlated with each other, we can now use the Chernoff bound.

	\begin{align*}
		Pr\bigg[\frac{deg_H(v)}{b_v}>(1+\epsilon)E_v\bigg] \leq exp\big(-\frac{\epsilon E_v}{2}\big) \enspace .
	\end{align*}

	Choosing $\epsilon = c\,log^2(n)/E_v$ for some constant $c$ shows that this probability can be as small as $O(1/poly(n))$ while the degree is violated with an additive term of $O(log^2(n))$. Moreover, it can be shown using union bound that the probability of any of the vertices being violated is low enough ($O(1/poly(n))$).

	For the weight constraint let $X_e$ be a random variable which is $w(e)/w(opt)$ if $e\in H$, and zero otherwise. Note that in solving \ref{LP_scaled_primal} we assume that we are given $w(opt)$. Hence, we discard all edges with weight larger than $w(opt)$. This does not affect the analysis of the fractional solution. Now every random variable $X_e$ is between zero and one. 

	\begin{align*}
		E\bigg[\frac{w(H)}{w(opt)}\bigg] = E\bigg[\sum_{e\in E} X_e\bigg] = \sum_{e\in E} \bigg (\frac{w(e)}{w(opt)}Pr[X_e=1]\bigg) &= \sum_{e\in E}\bigg(\frac{w(e)}{w(opt)}\sum_{P_{i,j}:e\in P_{i,j}}f(P_{i,j})\bigg) \\
		&\leq \sum_{e\in E}\bigg(\frac{w(e)}{w(opt)}\sum_{i=1}^{|\sigma|}x_{e}^{i}\bigg) \in O(log^2(n))
	\end{align*}

\end{proof}

%Note that this set of covering constraints includes only variables of type $x_{e}^{i}$ for some $e\in E$. After 

==> perliminaries.tex <==
\section{Preliminaries}
In this section we formally define the stochastic $k$-server problem. The classical $k$-server problem is defined on a metric $\metric$ which is consisted of points that could be infinitely many. For every two points $x$ and $y$ in metric $\metric$, let $d(x,y)$ denote the distance of $x$ from $y$ which is a symmetric function and satisfies the triangle inequality. More precisely for every three points $x$, $y$, and $z$ we have
\begin{equation}
d(x,x) = 0
\end{equation}
\begin{equation}
d(x,y) = d(y,x)
\end{equation}
\begin{equation}
d(x,y) + d(y,z) \geq d(x,z).
\end{equation}
In the $k$-server problem the goal is to place $k$ servers on $k$ points of the metric, and move these servers to satisfy the requests. We refer to every placement of the servers on the metric points by a \textit{configuration}. Let $\req = \langle r_1,r_2,\ldots,r_t\rangle$ be a sequence of requests, the goal of the $k$-server problem is to find configurations $\langle A_0,A_2,\ldots,A_t\rangle$ such that for every $i$ there exists a server on point $r_i$ in configuration $A_i$. We say such a list of configurations is \textit{valid} for the given list of requests. A valid sequence of configurations is optimal if $\sum d(A_{i-1},A_i)$ is minimized where $d(X,Y)$ stands for the minimum cost of moving servers from configuration $X$ to configuration $Y$. An optimal sequence $\langle A_0,A_2,\ldots,A_t\rangle$ of configurations is called an optimal offline solution of $\KO(\metric,\req)$ when $\req$ is known in advance. We refer to the optimal cost of such movements with $|\KO(\metric,\req)| = \sum d(A_{i-1},A_i)$. 

We also define the notion of \textit{fractional configuration} as an assignment of the metric points to non-negative real numbers. More precisely, each number specifies a mass of fractional server on a point. Every fractional solution adheres to the following condition: The total sum of the values assigned to all points is exactly equal to $k$. Analogously, a fractional configuration serves a request $r_i$ if there is a mass of size at least 1 of server assigned to point $r_i$. An offline fractional solution of the $k$-server problem for a given sequence of requests $\rho$ is defined as a sequence of fractional configurations $\langle A_0, A_1, \ldots, A_t\rangle$ such that every $A_i$ serves $r_i$.
 
In the online $k$-server problem, however, we're not given the whole sequence of requests in the beginning, but we will be informed of every request once it is realized. An algorithm $\A$ is an online algorithm for the $k$-server problem if it reports a configuration $A_0$ as an initial configuration and upon realization of every request $r_i$ it returns a configuration $A_i$ such that $\langle A_0, A_1, A_2, \ldots, A_i\rangle$ is valid for $\langle r_1,r_2,\ldots,r_i\rangle$. If $\A$ is deterministic, it generates a unique sequence of configurations for every sequence of requests. Let $\A(\metric,\req)$ be the sequence that $\A$ generates for requests in $\req$ and $|\A(\metric,\req)|$ denote its cost. %We similarly denote the expected cost of a randomized algorithm $\A$ for a given request $\req$ with metric $\metric$ by $|\A(\metric,\req)|$.


In the online stochastic $k$-server problem, in addition to metric $\metric$, we are also given  $t$ independent probability distributions $\langle P_1,P_2,\ldots,P_t \rangle$ which show the probability that every request $r_i$ is realized on a point of the metric at each time. An algorithm $\A$ is an online algorithm for such a setting, if it generates a configuration for every request $r_i$ not solely based on $\langle r_1, r_2, \ldots, r_i\rangle$ and $\langle A_0, A_1, \ldots, A_{i-1}\rangle$ but also with respect to the probability distributions. Similarly, we define the cost of an online algorithm $\A$ for a given sequence of requests $\req$ with $|\A(\metric,\req,\langle P_1, P_2, \ldots, P_t\rangle)|$. We define the expected cost of an algorithm $\A$ on metric $\metric$ and with probability distributions $\langle P_1, P_2, \ldots, P_t\rangle$ by 
\begin{equation*}
|\A(\metric,\langle P_1, P_2, \ldots, P_t\rangle)| = \mathbb{E}_{\forall i, r_i \sim P_i} |\A(\metric,\req,\langle P_1,P_2,\ldots,P_t \rangle)|.
\end{equation*}
For every metric $\metric$ and probability distributions $\langle P_1, P_2, \ldots, P_t\rangle$ we refer to the online algorithm with the minimum cost by $\OPT_{\metric,\langle P_1, P_2, \ldots, P_t\rangle}$.

An alternative way to represent a solution of the $k$-server problem is as a vector of configurations $\langle B_0, B_1, \ldots, B_t \rangle$ such that $B_i$ does not necessarily serve request $r_i$. The cost of such solution is equal to $\sum d(B_{i-1},B_i) + \sum 2  d(B_i, r_i)$ where $d(B_i, r_i)$ is the minimum distance of a server in configuration $B_i$ to request $r_i$. The additional cost of $2 d(B_i, r_i)$ can be thought of as moving a server from $B_i$ to serve $r_i$ and returning it back to its original position. Thus, every such representation of a solution can be transformed to the other representation. Similarly, $d(B_i, r_i)$ for a fractional configuration $B_i$ is the minimum cost which is incurred by placing a mass 1 of server at point $r_i$. We use letter $B$ for the configurations of such solutions throughout the paper.

In this paper the emphasis is on the stochastic $k$-server problem on the line metric. We define the line metric $\Line$ as a metric of points from $-\infty$ to $+\infty$ such that the distance of two points $x$ and $y$ is always equal to $|x-y|$. Moreover, it is easy to show that deterministic algorithms are as powerful as the randomized algorithms in this setting, therefore we only focus on deterministic algorithms in this paper. Thus, from here on, we omit the term deterministic and every time we use the word algorithm we mean a deterministic algorithm unless otherwise is explicitly mentioned.

==> proofoflmaux.tex <==
Without loss of generality we assume that the tree is rooted at some vertex. We define the weight of every vertex as the number of vertices in its subtree including itself. Let $v$ be a vertex with the highest depth that has a weight of at least $\lfloor \frac{1}{3} |V(T)| \rfloor$. If we remove vertex $v$ and all the edges incident to $v$ from the tree, none of the remaining connected components would have a size more than $\lceil \frac{2}{3} |V(T)|\rceil + 1 $. 

Now, we start with an empty set $X$ and greedily add the vertices of the connected components to $X$ in descending order of their size until $|X|$ reaches $\lfloor \frac{1}{3} |V(T)| \rfloor$. Therefore $|X|$ contains at least $\lfloor \frac{1}{3} |V(T)| \rfloor$ vertices but its size is no more $\lceil \frac{2}{3} |V(T)|\rceil$. We define $T_1$ as the induced subgraph of $T$ on $\{v\} \cup X$ and $T_2$ as the induced subgraph of $T$ on $V(T) \setminus X$. Since $\lfloor \frac{1}{3} |V(T)| \rfloor \leq |X| \leq \lceil \frac{2}{3} |V(T)|\rceil$ we have $\max\{|V(T_1)|,|V(T_2)|\} \leq \lceil \frac{2}{3} |V(T)|\rceil + 1 $ and both $T_1$ and $T_2$ are trivially connected. Moreover $V(T_1) \cap V(T_2) = \{v\}$ and thus the proof is complete.


==> proofoflmsf1.tex <==
	We construct a solution $\{\x', \alpha\}$ from $\{\x, \alpha\}$ as follows. Let $x'_e=1$ if and only if there exists a subgraph $H$ and $1 \leq i \leq k$, such that $x_H^i=1$. For every vertex $v$, $\sum_{e \in \delta(v)}x'_e \leq \sum_{i=1}^k\sum_{H \subseteq G}\deg_H(v)x_H^i$. Moreover, $\sum_{e \in E}w(e)x'_e \leq \sum_{i=1}^k\sum_{H \subseteq G}w(H)x_H^i$. Thus each packing constraint in \ref{IP:sf} is satisfied. Hence it remains to prove every covering constraint in \ref{IP:sf} is also satisfied. We use an induction on the number of demands.
	
	For the first demand we know $\mathcal{H}_1$ is the set of subgraphs in which $s_1$ and $t_1$ are connected. Since $\x$ is feasible for \ref{IP:good}, there exists an $H \in \mathcal{H}_1$ such that $x_H^1=1$. Thus for each $e \in H$, $x'_e=1$ and therefore the hypothesis holds for the base case. Now we assume the first $l-1$ covering constraints are satisfied, i.e. for each demand $1 \leq i < l$ and set of vertices $S \subseteq V$ which separates $s_i$ and $t_i$, there exists an edge $e \in \delta(S)$ such that $x'_e=1$. In other words there exists a path from $s_i$ to $t_i$. We prove $\x'$ satisfies the $l$-th covering constraint as well. By contradiction assume there exists a set $S \subseteq V$ such that $S$ separates $s_l$ from $t_l$ and there exists no edge $e \in \delta(S)$ with $x'_e=1$. By induction hypothesis $S$ does not separate any of the first $l-1$ demands endpoints. Since otherwise there exists an edge $e\in \delta(S)$ such that $x'_e=1$. Thus for each demand $i<l$, $s_i$ and $t_i$ are either in $S$ or $V\setminus S$. On the other hand, there exists a path from $s_l$ to $t_l$ in subgraph $H_l\cup R_\sigma(l)$. Thus there exists a subgraph $H$ such that $x_H^l=1$ and for every set $S \subseteq V$ that separates $s_l$ from $t_l$ and does not separate any of the first $l-1$ demands endpoints, there exists an edge $e \in \delta(S)$ such that $e \in H$. Hence $x'_e=1$, which is a contradiction. Therefore $\{\x', \alpha\}$ is a feasible solution for \ref{IP:sf}.


==> proofofmain.tex <==
Here we give a sketch of the proof of lemma; we refer the reader to the appendix for detailed proofs.
We first prove a cost-minimization variant of the lemma.
%Recall that in \ref{IP:good}, we satisfy the $i^{th}$ demand $(s_i,t_i)$ by choosing a subgraph $Q_i\in \Mc{H}_i$.
Consider an arbitrary weight vector $\hat{w} : F\to \mathbb{R}^{\geq 0}$. We argue that there is a connective list $Q$, such that $\sum_i \hat{w}(Q_i)\leq O(\log^2 n) \hat{w}(F)$. Let $\hat{H}_i=(V,F\cup R_\sigma(i),\hat{w}_i)$ denote a weighted graph for which $\hat{w}_i(e)=\hat{w}(e)$ for $e\in F$, and $\hat{w}_i(e)=0$ for $e\in R_\sigma(i)$. Now we note that there is no cost-sharing among $Q_i$'s in the goal $\sum_i \hat{w}(Q_i)$. Therefore the optimal choice for $Q_i$ corresponds to the minimum-weight $(s_i,t_i)$-path in $\hat{H}_{i-1}$. Hence, we need to analyze the cost of these greedy choices.

Awerbuch et al.~\cite{AAB96} showed that the greedy algorithm is indeed $O(\log^2 n)$-competitive for the edge-weighted Steiner forest problem. The standard greedy algorithm is slightly different from the greedy process we discussed above. In the greedy algorithm of Awerbuch et al., at time step $i$ we choose a minimum-cost $(s_i,t_i)$-path in a graph in which there is a zero-cost edge between \textit{any} pair of vertices in the same connected component of the current solution; not just the $(s_j,t_j)$ pairs of the previous demands. However, in their analysis they only use the zero-cost edges among the terminals of a previous demand. This is indeed not surprising since we hardly have any control on the greedy choices other than the fact that they satisfy the demands. Therefore the following claim follows from the result of Awebuch et al.:

\begin{claim}[implicitly proven in Theorem 2.1 of \cite{AAB96}]\label{claim:greedy}
	For any weight function $\hat{w}$ defined over $F$, there exists a connective list $Q$ for which
	$$\sum_i \hat{w}(Q_i)\leq O(\log^2 n) \hat{w}(F)$$.
\end{claim}

\begin{remark}
	There is also a lower bound of $\Omega(\log n)$ for the competitive ratio of the greedy algorithm. Closing the gap between this lower bound and the upper bound of $O(\log^2 n)$ for EW Steiner forest is an important open problem.
\end{remark}

However, Claim~\ref{claim:greedy} is not enough for us. We need a solution in which every edge is used at most $O(\log^2 n)$ times, not just in an amortized sense. Next in Lemma~\ref{mohem}, we show that since there is a solution for \textit{every} weight function, we can have a \textit{fractional} connecting list $Q$ in which every edge is used (fractionally) at most $O(\log^2 n)$ times. Indeed, Lemma~\ref{mohem} can be proven for a far more general setting, which might be of its own interest: the same argument fundamentally holds for any arbitrary combinatorial problem for which the feasible space can be described by a convex polytope. We refer the reader to Section~\ref{sec:redavglemma} for further discussion.

Claim~\ref{claim:greedy} and Lemma~\ref{mohem} imply that we have a fractional connecting list. Finally in Section~\ref{sec:rounding}, we provide a rounding argument which obtains an integral connecting list by losing only a constant factor; which completes the proof of lemma. 





%We prove this lemma by an induction on $|E(F)|$. 
%The base case is when $|E(F)| \leq 2$ for which the proof is trivial.
%Now we assume the hypothesis of the induction holds for all forests $F$ such that $|E(F)| < n$ and we prove it for the case of $|E(F)| = n$.\\
%If the forest is not connected, then by the hypothesis of the induction, the lemma holds for each connected component and hence it holds for the whole forest. Therefore, without loss of generality, we assume $F$ is a tree. According to Lemma \ref{aux} we can decompose $F$ into two trees $T_1$ and $T_2$ sharing a single vertex and no edges. Now we create two separate lists $\sigma_1$ and $\sigma_2$ in the following way:
%We start from $i = 1$ and iterate through all pairs of $\sigma$. For each pair $(s_i, t_i)$ we do the following
%\begin{enumerate}
%	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we add pair $(s_i, t_i)$ to $\sigma_1$.
%	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we add pair $(s_i, t_i)$ to $\sigma_2$.
%	\item Otherwise, without loss of generality we assume $s_i \in V(T_1)$ and $t_i \in V(T_2)$ and do the following
%	\begin{enumerate}
%	\item If $(s_i,t_i)$ is the first of such pairs, we do nothing.
%	\item If $(s_i,t_i)$ is not the first pair of this type, we add pair $(s_i,s_x)$ to $\sigma_1$ and $(t_i,t_x)$ to $\sigma_2$ where $(s_x,t_x)$ is the first pair with this condition.
%	\end{enumerate}
%\end{enumerate}
%
%Now, by the hypothesis of the induction we can find connective subgraphs $Q^1 = \langle Q^1_1, Q^1_2, \ldots, Q^1_{|\sigma_1|} \rangle$ and $Q^2 = \langle Q^2_1, Q^2_2, \ldots, Q^2_{|\sigma_2|} \rangle$ for instances of the problem $\langle G, T_1, \sigma_1\rangle$ and $\langle G, T_2, \sigma_2\rangle$ meeting the constraints of the lemma. Next, we create a list of connective subgraphs $Q$ for $\langle G, F, \sigma\rangle$ as follows. For every pair $(s_i, t_i) \in \sigma$ we do the following:
%\begin{enumerate}
%	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^1$.
%	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^2$.
%	\item If not both of $s_i$ and $t_i$ are in one of the trees:
%	\begin{enumerate}
%		\item If $s_i$ and $t_i$ are the first of such pairs, we set $Q_i$ to be the union of the edges in the path from $s_i$ to $t_i$ .
%		\item Otherwise let $(s_i,s_x)$ and $(t_i,t_x)$ be the pairs in $\sigma_1$ and $\sigma_2$ associated to $(s_i,t_i)$. We set $Q_i$ to be the union of the subgraphs corresponding $(s_i,s_x)$ and $(t_i,t_x)$ in $Q^1$ and $Q^2$.
%	\end{enumerate}
%\end{enumerate}
%Note that, by the hypothesis of induction every edge appears in no more than $3 \log (\lceil \frac{2}{3} |V(F)|\rceil+1) \leq 3 \log n - 1$ sets of $Q_1$ and $Q_2$. Apart from the edges of $Q_1$ and $Q_2$, the only new edges in $Q$ are the ones in the path from $s_x$ to $t_x$ that goes through every edge at most once. Therefore, every edge of the graph appears in at most $3 \log n $ subgraphs of $Q$. In the rest we argue that $Q$ is a connective list of subgraphs for $\langle G, F, \sigma\rangle$.
%
%Note that the conditions of the lemma hold for all pairs of vertices $(s_i, t_i)$ that completely lie in one of the trees. Moreover, for the first $(s_x, t_x)$ that is separated by the trees, the conditions are also satisfied since $Q_i$ is a path from $s_x$ to $t_x$ and therefore no disjoint cut from $Q_i$ can separate $s_x$ from $t_x$. All that remains is to show the same properties for the rest of such pairs.  Let $(s_i, t_i)$ be a pair which is separated by the trees and $i > x$. If a cut $c$ disjoint from $Q_i$ separates $s_i$ from $t_i$ and not $s_x$ from $t_x$, then either of $s_i$ or $t_i$ should be separated from both $s_x$ and $t_x$. However, this leads to contradiction because this is guaranteed to not happen due to our construction of $Q_i$ and the fact that both $Q^1$ and $Q^2$ are connective list of subgraphs for $\langle G, T_1, \sigma_1\rangle$ and $\langle G, T_2, \sigma_2\rangle$.


==> proofofmain_-_Copy.tex <==
Here we give a sketch of the proof of lemma; we refer the reader to the appendix for detailed proofs.
We first prove a cost-minimization variant of the lemma.
%Recall that in \ref{IP:good}, we satisfy the $i^{th}$ demand $(s_i,t_i)$ by choosing a subgraph $Q_i\in \Mc{H}_i$.
Consider an arbitrary weight vector $\hat{w} : F\to \mathbb{R}^{\geq 0}$. We argue that there is a connective list $Q$, such that $\sum_i \hat{w}(Q_i)\leq O(\log^2 n) \hat{w}(F)$. Let $\hat{G}_i=(V,E\cup R_\sigma(i),\hat{w}_i)$ denote a weighted graph for which $\hat{w}_i(e)=\hat{w}(e)$ for $e\in E$, and $\hat{w}_i(e)=0$ for $e\in R_\sigma(i)$. Now we note that there is no cost-sharing among $Q_i$'s. Therefore the optimal choice for $Q_i$ corresponds to the minimum-cost $(s_i,t_i)$-path in $\hat{G}_{i-1}$. Hence, we need to analyze the cost of these greedy choices.

Awerbuch et al.~\cite{AAB96} showed that the greedy algorithm is indeed $O(\log^2 n)$-competitive for the edge-weighted Steiner forest problem. The standard greedy algorithm is slightly different from the greedy process we discussed above. In the greedy algorithm of Awerbuch et al., at time step $i$ we choose a minimum-cost $(s_i,t_i)$-path in a graph in which there is a zero-cost edge between \textit{any} pair of vertices in the same connected component of the current solution; not just the $(s_j,t_j)$ pairs of the previous demands. However, in their analysis they only use the zero-cost edges among the terminals of a previous demand. This is indeed not surprising since we hardly have any control on the greedy choices other than the fact that they satisfy the demands. Therefore the following theorem follows from the result of Awebuch et al.:

\begin{theorem}[implicitly proven in Theorem 2.1 of \cite{AAB96}]
	For any weight function $\hat{w}$ defined over the edges, there exists a sequence of subgraphs $Q_i\in \Mc{H}_i$ satisfying demands for which
	$$\sum_i \hat{w}(Q_i)\leq O(\log^2 n) \lpopt(\hat{w})$$.
\end{theorem}

\begin{remark}
	There is also a lower bound of $\Omega(\log n)$ for the competitive ratio of the greedy algorithm. Closing the gap between this lower bound and the upper bound of $O(\log^2 n)$ for EW Steiner forest is an important open problem.
\end{remark}





%We prove this lemma by an induction on $|E(F)|$. 
%The base case is when $|E(F)| \leq 2$ for which the proof is trivial.
%Now we assume the hypothesis of the induction holds for all forests $F$ such that $|E(F)| < n$ and we prove it for the case of $|E(F)| = n$.\\
%If the forest is not connected, then by the hypothesis of the induction, the lemma holds for each connected component and hence it holds for the whole forest. Therefore, without loss of generality, we assume $F$ is a tree. According to Lemma \ref{aux} we can decompose $F$ into two trees $T_1$ and $T_2$ sharing a single vertex and no edges. Now we create two separate lists $\sigma_1$ and $\sigma_2$ in the following way:
%We start from $i = 1$ and iterate through all pairs of $\sigma$. For each pair $(s_i, t_i)$ we do the following
%\begin{enumerate}
%	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we add pair $(s_i, t_i)$ to $\sigma_1$.
%	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we add pair $(s_i, t_i)$ to $\sigma_2$.
%	\item Otherwise, without loss of generality we assume $s_i \in V(T_1)$ and $t_i \in V(T_2)$ and do the following
%	\begin{enumerate}
%	\item If $(s_i,t_i)$ is the first of such pairs, we do nothing.
%	\item If $(s_i,t_i)$ is not the first pair of this type, we add pair $(s_i,s_x)$ to $\sigma_1$ and $(t_i,t_x)$ to $\sigma_2$ where $(s_x,t_x)$ is the first pair with this condition.
%	\end{enumerate}
%\end{enumerate}
%
%Now, by the hypothesis of the induction we can find connective subgraphs $Q^1 = \langle Q^1_1, Q^1_2, \ldots, Q^1_{|\sigma_1|} \rangle$ and $Q^2 = \langle Q^2_1, Q^2_2, \ldots, Q^2_{|\sigma_2|} \rangle$ for instances of the problem $\langle G, T_1, \sigma_1\rangle$ and $\langle G, T_2, \sigma_2\rangle$ meeting the constraints of the lemma. Next, we create a list of connective subgraphs $Q$ for $\langle G, F, \sigma\rangle$ as follows. For every pair $(s_i, t_i) \in \sigma$ we do the following:
%\begin{enumerate}
%	\item If both $s_i$ and $t_i$ are in $V(T_1)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^1$.
%	\item If both $s_i$ and $t_i$ are in $V(T_2)$, we set $Q_i$ to be the subgraph of its corresponding pair in $Q^2$.
%	\item If not both of $s_i$ and $t_i$ are in one of the trees:
%	\begin{enumerate}
%		\item If $s_i$ and $t_i$ are the first of such pairs, we set $Q_i$ to be the union of the edges in the path from $s_i$ to $t_i$ .
%		\item Otherwise let $(s_i,s_x)$ and $(t_i,t_x)$ be the pairs in $\sigma_1$ and $\sigma_2$ associated to $(s_i,t_i)$. We set $Q_i$ to be the union of the subgraphs corresponding $(s_i,s_x)$ and $(t_i,t_x)$ in $Q^1$ and $Q^2$.
%	\end{enumerate}
%\end{enumerate}
%Note that, by the hypothesis of induction every edge appears in no more than $3 \log (\lceil \frac{2}{3} |V(F)|\rceil+1) \leq 3 \log n - 1$ sets of $Q_1$ and $Q_2$. Apart from the edges of $Q_1$ and $Q_2$, the only new edges in $Q$ are the ones in the path from $s_x$ to $t_x$ that goes through every edge at most once. Therefore, every edge of the graph appears in at most $3 \log n $ subgraphs of $Q$. In the rest we argue that $Q$ is a connective list of subgraphs for $\langle G, F, \sigma\rangle$.
%
%Note that the conditions of the lemma hold for all pairs of vertices $(s_i, t_i)$ that completely lie in one of the trees. Moreover, for the first $(s_x, t_x)$ that is separated by the trees, the conditions are also satisfied since $Q_i$ is a path from $s_x$ to $t_x$ and therefore no disjoint cut from $Q_i$ can separate $s_x$ from $t_x$. All that remains is to show the same properties for the rest of such pairs.  Let $(s_i, t_i)$ be a pair which is separated by the trees and $i > x$. If a cut $c$ disjoint from $Q_i$ separates $s_i$ from $t_i$ and not $s_x$ from $t_x$, then either of $s_i$ or $t_i$ should be separated from both $s_x$ and $t_x$. However, this leads to contradiction because this is guaranteed to not happen due to our construction of $Q_i$ and the fact that both $Q^1$ and $Q^2$ are connective list of subgraphs for $\langle G, T_1, \sigma_1\rangle$ and $\langle G, T_2, \sigma_2\rangle$.


==> reduction_fractional.tex <==
\section{Reduction From Integral $k$-server to Fractional $k$-server}\label{fred}
In this section we show how we can obtain an integral algorithm for the stochastic $k$-server problem from a fractional algorithm. We first show that every fractional algorithm for the line metric can be modified to an integral algorithm with the same cost. Next, we study the problem on HST metrics; we give a rounding method that produces an integral algorithm from a fractional algorithm while losing a constant factor. Finally, we leverage the previously known embedding techniques to show every metric can be embedded into HST's with a distortion of at most $O(\log n)$. This will lead to a rounding method for obtaining an integral algorithm from every fractional algorithm on general metrics while losing a factor of at most $O(\log n)$. Combining this with the $3$ approximation fractional algorithm that we provide in Section \ref{fsf}, we achieve an $O(\log n)$ approximation algorithm for the stochastic $k$-server problem on general graphs. 
\input{line_reduction}
\input{hst_reduction}
%\input{general_graph_to_hst}

==> structural_characterization.tex <==
\section{Structural Characterization}
In this section we define a class of online algorithms for the stochastic $k$-server problem and show an important structural property for this class. Later, we leverage this property to provide a polynomial time algorithm for the problem. Although we give the algorithm for the line metric, the structural characterization holds for general graphs and is of independent interest.

Recall that an online algorithm $\A$ has to fulfill the task of reporting a configuration $A_i$ upon arrival of request $r_i$ based on $\langle A_0, A_1, \ldots, A_{i-1} \rangle$, $\langle r_1, r_2, \ldots, r_i\rangle$, and $\langle P_1, P_2, \ldots, P_t\rangle$. We say an algorithm $\B$ is \textit{request oblivious}, if it reports  configuration $B_i$ regardless of request $r_i$. As such, $\B$ generates configurations $\langle B_0, B_1, \ldots, B_t\rangle$ for a sequence of requests $\langle r_1, r_2, \ldots, r_t\rangle$ and the cost of such configuration is $\sum d(B_{i-1},B_i) + \sum 2  d(B_i, r_i)$. More precisely, no matter what request $r_i$ is, $\B$ will generate the same configuration for a given list of past configurations $\langle B_0, B_1, \ldots, B_{i-1}\rangle$, a given sequence of past requests $\langle r_1, r_2, \ldots, r_{i-1}\rangle$, and the sequence of probability distributions $\langle P_1, P_2, \ldots, P_t\rangle$. In the following we show that every online algorithm $\A$ can turn into a request oblivious algorithm $\B_{\A}$ that has a cost of at most $|3\A(\metric,\req,\langle P_1, P_2, \ldots, P_t\rangle)|$ for a given sequence of requests $\req$.
\begin{lemma}\label{lm1}
Let $\A$ be an online algorithm for the stochastic $k$-server problem. For any matric $\metric$, there exists a request oblivious algorithm $\B_{\A}$ such that $$|\B_{\A}(\metric,\langle P_1, P_2, \ldots, P_t\rangle)| \leq 3|\A(\metric,\langle P_1, P_2, \ldots, P_t\rangle)|.$$
\end{lemma}
\begin{proof}
Let $\req$ be a sequence of requests. We define online algorithm $\B_{\A}$ as follows: The configuration that $\B_{\A}$ reports for a given list of input arguments $\langle B_0, B_1, \ldots, B_i \rangle$, $\langle r_1, r_2, \ldots, r_i\rangle$, and $\langle P_1, P_2, \ldots, P_t\rangle$ is the output of algorithm $\A$ on inputs $\langle B_0, B_1, \ldots, B_i \rangle$, $\langle r_1, r_2, \ldots, r_{i-1}\rangle$, and $\langle P_1, P_2, \ldots, P_t\rangle$ (The same input except that $r_i$ is dropped from the sequence of requests). We show the cost of such algorithm for input $\req$ is at most 3 times the cost of $\A$ for the same input.

Let $\langle A_0, A_1, \ldots, A_t\rangle$ be the sequence of configurations that $\A$ generates for requests $\req$ and $\langle B_0, B_1, \ldots, B_t\rangle$ be the output of algorithm $\B_{A}$. According to the construction of $\B_{\A}$, $B_0 = A_0$ and $B_i = A_{i-1}$ for all $1 \leq i \leq t$. Note that for algorithm $\A$, we assume every $A_i$ serves request $r_i$. By definition, the cost of solution $\langle B_0, B_1, B_2, \ldots, B_t\rangle$ is equal to $\sum d(B_{i-1},B_i) + 2\sum d(B_i, r_i)$. Since $B_0 = B_1 = A_0$ and $B_i$ = $A_{i-1}$, 
\begin{equation}\label{cc1}
\sum_{i=1}^{t} d(B_{i-1},B_i) = \sum_{i=1}^{t-1} d(A_{i-1},A_i) \leq \sum_{i=1}^t d(A_{i-1},A_i) = |\A(\metric, \req, \langle P_1, P_2, \ldots, P_t\rangle)|.
\end{equation}
Moreover, since every $A_i$ servers request $r_i$, $d(B_i,r_i) \leq d(B_i, A_i) = d(A_{i-1},A_i)$. Hence,
\begin{equation}\label{cc2}
2\sum_{i=1}^t d(B_i, r_i) \leq 2\sum_{i=1}^t d(B_i, A_i) = 2\sum_{i=1}^t d(A_{i-1},A_i) = 2|\A(\metric,\req,\langle P_1, P_2, \ldots, P_t\rangle)|.
\end{equation}
Inequality \eqref{cc1} along with Equation \eqref{cc2} implies $$|\B_\A(\metric,\req,\langle P_1, P_2, \ldots, P_t\rangle)| \leq 3|\A(\metric,\req,\langle P_1, P_2, \ldots, P_t\rangle)|.$$
Since this holds for all requests $\req \sim \langle P_1, P_2, \ldots, P_t\rangle$, we have $$|\B_\A(\metric,\langle P_1, P_2, \ldots, P_t\rangle)| \leq 3|\A(\metric, \langle P_1, P_2, \ldots, P_t\rangle)|$$ and the proof is complete.
\end{proof}

An immediate corollary of Lemma \ref{lm1} is that the optimal request oblivious algorithm has a cost of at most $|3\OPT_{\metric,\langle P_1, P_2, \ldots, P_t\rangle}(\metric, \langle P_1, P_2, \ldots, P_t\rangle)|$. Therefore, if we only focus on the request oblivious algorithms, we only lose a factor of 3 in comparison to the optimal online algorithm. The following lemma states a key structural lemma for an optimal request oblivious algorithm.

\begin{lemma}\label{mohem}
For every request oblivious algorithm $\B$, there exists a randomized request oblivious algorithm $\B'$ with the same expected cost which is not only oblivious to the last request, but also oblivious to all requests that have come prior to this.
\end{lemma}
\begin{proof}
For any given request oblivious online algorithm $\B$, we construct an online algorithm $\B'$ which is oblivious to all of the requests as follows: For an input $\langle B_1, B_2, \ldots, B_{i-1}\rangle$ of configurations and probability distributions $\langle P_1, P_2, \ldots, P_t\rangle$, draw a sequence of requests $\langle r_1, r_2, \ldots, r_i\rangle$ from $\langle P_1, P_2, \ldots, P_t\rangle$ conditioned on the constraint that $\B$ would generate configurations $\langle B_1, B_2, \ldots, B_{i-1}\rangle$ for requests $\langle r_1, r_2, \ldots, r_{i-1}\rangle$. Now, report the output of $\B$ for inputs $\langle B_1, B_2, \ldots, B_{i-1}\rangle$, $\langle r_1, r_2, \ldots, r_i\rangle$, and $\langle P_1, P_2, \ldots, P_t\rangle$.

We define the cost of step $i$ of Algorithm $B'$ as $d(B_{i-1},B_{i}) + 2d(B_i,r_i)$. Due to the construction of algorithm $\B'$, the expected cost of this algorithm at every step $i$ for a random sequence of requests is equal to the expected cost of algorithm $\B$ for a random sequence of requests drawn from $\langle P_1, P_2, \ldots, P_t\rangle$. Therefore, the expected cost of both algorithms for a random sequence of requests are equal and thus $|\B(\metric,\langle P_1, P_2, \ldots, P_t\rangle)| = |\B'(\metric,\langle P_1, P_2, \ldots, P_t\rangle)|$.
\end{proof}

Lemma \ref{mohem} states that there always exists an optimal randomized request oblivious online algorithm that returns the configurations regardless of the requests. We call such an algorithm \textit{non-adaptive}. Since a non-adaptive algorithm is indifferent to the sequence of the requests, we can assume it always generates a sequence of configurations just based on the distributions. For an optimal of such algorithms, all such sequence of configurations should be optimal as well. Therefore, there always exists an optimal non-adaptive online algorithm which is deterministic. By Lemma \ref{lm1} not only do we know the optimal request oblivious algorithm is at most 3-approximation, but also the same holds for the optimal non-adaptive algorithm. 
\begin{theorem}\label{thebest}
There exists a sequence of configurations $\langle B_0, B_1, \ldots, B_t\rangle$ such that an online algorithm which starts with $B_0$ and always returns configuration $B_i$ upon arrival of request $r_i$ has an opproximation factor of at most 3. 
\end{theorem}

==> structural_lemma.tex <==
\section{Structural Characterization}
